Reliability Assurance for Deep Neural Network Architectures Against Numerical Defects

With the widespread deployment of deep neural networks (DNNs), ensuring the reliability of DNN-based systems is of great importance. Serious reliability issues such as system failures can be caused by numerical defects, one of the most frequent defects in DNNs. To assure high reliability against numerical defects, in this paper, we propose the RANUM approach including novel techniques for three reliability assurance tasks: detection of potential numerical defects, confirmation of potential-defect feasibility, and suggestion of defect fixes. To the best of our knowledge, RANUM is the first approach that confirms potential-defect feasibility with failure-exhibiting tests and suggests fixes automatically. Extensive experiments on the benchmarks of 63 real-world DNN architectures show that RANUM outperforms state-of-the-art approaches across the three reliability assurance tasks. In addition, when the RANUM-generated fixes are compared with developers' fixes on open-source projects, in 37 out of 40 cases, RANUM-generated fixes are equivalent to or even better than human fixes.

==> exp/tables/detect_table.tex <==


\begin{table}[!t]
    \centering
    \caption{(RQ1) Defect detection result for \sysname~(``R'' column) and DEBAR~\cite{zhang2020detecting}~(``D'' column). 
    % Statistics for DEBAR are digested from \cite{yan2021exposing}. 
    ``\checkmark'' means the numerical defect is detected; otherwise ``$\times$''.
    \sysname detects defects in all cases.
    % All approaches are deterministic and finish in \SI{3}{s} per case.
    }
    \vspace{-1.0em}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{ccc|ccc|ccc|ccc|ccc}
        \toprule
        Case & \multirow{2}{*}{\textbf{R}} & \multirow{2}{*}{D} & 
        Case & \multirow{2}{*}{\textbf{R}} & \multirow{2}{*}{D} & 
        Case & \multirow{2}{*}{\textbf{R}} & \multirow{2}{*}{D} & 
        Case & \multirow{2}{*}{\textbf{R}} & \multirow{2}{*}{D} & 
        Case & \multirow{2}{*}{\textbf{R}} & \multirow{2}{*}{D} \\
        ID & & &
        ID & & &
        ID & & &
        ID & & &
        ID & & \\
        \hline

1 & $\checkmark$ & $\checkmark$ & 13 & $\checkmark$ & $\times$ & 27 & $\checkmark$ & $\times$ & 38 & $\checkmark$ & $\times$ & 49b & $\checkmark$ & $\times$ \\
2a & $\checkmark$ & $\checkmark$ & 14 & $\checkmark$ & $\checkmark$ & 28a & $\checkmark$ & $\checkmark$ & 39a & $\checkmark$ & $\checkmark$ & 50 & $\checkmark$ & $\checkmark$ \\
2b & $\checkmark$ & $\checkmark$ & 15 & $\checkmark$ & $\checkmark$ & 28b & $\checkmark$ & $\checkmark$ & 39b & $\checkmark$ & $\times$ & 51 & $\checkmark$ & $\times$ \\
3 & $\checkmark$ & $\checkmark$ & 16a & $\checkmark$ & $\checkmark$ & 28c & $\checkmark$ & $\checkmark$ & 40 & $\checkmark$ & $\times$ & 52 & $\checkmark$ & $\checkmark$ \\
4 & $\checkmark$ & $\times$ & 16b & $\checkmark$ & $\checkmark$ & 28d & $\checkmark$ & $\checkmark$ & 41 & $\checkmark$ & $\times$ & 53 & $\checkmark$ & $\times$ \\
5 & $\checkmark$ & $\times$ & 16c & $\checkmark$ & $\checkmark$ & 29 & $\checkmark$ & $\checkmark$ & 42 & $\checkmark$ & $\times$ & 54 & $\checkmark$ & $\times$ \\
6 & $\checkmark$ & $\checkmark$ & 17 & $\checkmark$ & $\times$ & 30 & $\checkmark$ & $\checkmark$ & 43a & $\checkmark$ & $\checkmark$ & 55 & $\checkmark$ & $\checkmark$ \\
7 & $\checkmark$ & $\checkmark$ & 18 & $\checkmark$ & $\checkmark$ & 31 & $\checkmark$ & $\checkmark$ & 43b & $\checkmark$ & $\times$ & 56 & $\checkmark$ & $\times$ \\
8 & $\checkmark$ & $\checkmark$ & 19 & $\checkmark$ & $\checkmark$ & 32 & $\checkmark$ & $\times$ & 44 & $\checkmark$ & $\checkmark$ & 57 & $\checkmark$ & $\times$ \\
9a & $\checkmark$ & $\checkmark$ & 20 & $\checkmark$ & $\checkmark$ & 33 & $\checkmark$ & $\times$ & 45a & $\checkmark$ & $\checkmark$ & 58 & $\checkmark$ & $\checkmark$ \\
9b & $\checkmark$ & $\checkmark$ & 21 & $\checkmark$ & $\checkmark$ & 34 & $\checkmark$ & $\times$ & 45b & $\checkmark$ & $\checkmark$ & 59 & $\checkmark$ & $\checkmark$ \\
10 & $\checkmark$ & $\checkmark$ & 22 & $\checkmark$ & $\times$ & 35a & $\checkmark$ & $\checkmark$ & 46 & $\checkmark$ & $\times$ & 60 & $\checkmark$ & $\checkmark$ \\
11a & $\checkmark$ & $\checkmark$ & 23 & $\checkmark$ & $\times$ & 35b & $\checkmark$ & $\times$ & 47 & $\checkmark$ & $\times$ & 61 & $\checkmark$ & $\checkmark$ \\
11b & $\checkmark$ & $\checkmark$ & 24 & $\checkmark$ & $\checkmark$ & 36a & $\checkmark$ & $\checkmark$ & 48a & $\checkmark$ & $\checkmark$ & 62 & $\checkmark$ & $\times$ \\
11c & $\checkmark$ & $\checkmark$ & 25 & $\checkmark$ & $\checkmark$ & 36b & $\checkmark$ & $\times$ & 48b & $\checkmark$ & $\checkmark$ & 63 & $\checkmark$ & $\times$ \\
\cline{13-15}
12 & $\checkmark$ & $\times$ & 26 & $\checkmark$ & $\times$ & 37 & $\checkmark$ & $\times$ & 49a & $\checkmark$ & $\checkmark$ & \textbf{Tot} & \textbf{79} & \textbf{48} \\
    

        \bottomrule
    \end{tabular}
}
    \label{tab:detect}
    % \vspace{-1.0em}
\end{table}


% \begin{table*}[th]
%     \centering
%     \caption{(RQ4) Statistics for static defect detection for \sysname~(``Ours'' in table) and DEBAR~\cite{zhang2020detecting}~(``DB'' in table). Statistics for DEBAR are digested from \cite{yan2021exposing}. ``\checkmark'' means all numerical defects are detected, ``$\times$'' means not all, and ``?'' means unknown~(not reported in \cite{yan2021exposing}).
%     All approaches are deterministic and finish in \SI{3}{s} per case.}
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
%         \toprule
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} & 
%         Case & \multirow{2}{*}{Ours} & \multirow{2}{*}{DB} \\
%         ID & & &
%         ID & & &
%         ID & & &
%         ID & & &
%         ID & & &
%         ID & & &
%         ID & & &
%         ID & & &
%         ID & & &
%         ID & & &
%         ID & & \\
%         \hline
    
% 1 & $\checkmark$ & $\checkmark$ & 8 & $\checkmark$ & $\checkmark$ & 13 & $\checkmark$ & $\times$ & 19 & $\checkmark$ & $\checkmark$ & 27 & $\checkmark$ & $\times$ & 31 & $\checkmark$ & $\checkmark$ & 36b & $\checkmark$ & $\times$ & 41 & $\checkmark$ & $\times$ & 46 & $\checkmark$ & $\times$ & 51 & $\checkmark$ & $\times$ & 59 & $\checkmark$ & $\checkmark$ \\
% 2a & $\checkmark$ & $\checkmark$ & 9a & $\checkmark$ & $\checkmark$ & 14 & $\checkmark$ & $\checkmark$ & 20 & $\checkmark$ & $\checkmark$ & 28a & $\checkmark$ & $\checkmark$ & 32 & $\checkmark$ & $\times$ & 36c & $\checkmark$ & ? & 42 & $\checkmark$ & $\times$ & 47 & $\checkmark$ & $\times$ & 52 & $\checkmark$ & $\checkmark$ & 60 & $\checkmark$ & $\checkmark$ \\
% 2b & $\checkmark$ & $\checkmark$ & 9b & $\checkmark$ & $\checkmark$ & 15 & $\checkmark$ & $\checkmark$ & 21 & $\checkmark$ & $\checkmark$ & 28b & $\checkmark$ & $\checkmark$ & 33 & $\checkmark$ & $\times$ & 37 & $\checkmark$ & $\times$ & 43a & $\checkmark$ & $\checkmark$ & 48a & $\checkmark$ & $\checkmark$ & 53 & $\checkmark$ & $\times$ & 61 & $\checkmark$ & $\checkmark$ \\
% 3 & $\checkmark$ & $\checkmark$ & 10 & $\checkmark$ & $\checkmark$ & 16a & $\checkmark$ & $\checkmark$ & 22 & $\checkmark$ & $\times$ & 28c & $\checkmark$ & $\checkmark$ & 34 & $\checkmark$ & $\times$ & 38 & $\checkmark$ & $\times$ & 43b & $\checkmark$ & $\times$ & 48b & $\checkmark$ & $\checkmark$ & 54 & $\checkmark$ & $\times$ & 62 & $\checkmark$ & $\times$ \\
% 4 & $\checkmark$ & $\times$ & 11a & $\checkmark$ & $\checkmark$ & 16b & $\checkmark$ & $\checkmark$ & 23 & $\checkmark$ & $\times$ & 28d & $\checkmark$ & $\checkmark$ & 35a & $\checkmark$ & $\checkmark$ & 39a & $\checkmark$ & $\checkmark$ & 43c & $\checkmark$ & ? & 49a & $\checkmark$ & $\checkmark$ & 55 & $\checkmark$ & $\checkmark$ & 63 & $\checkmark$ & $\times$ \\
% \cline{31-33}
% 5 & $\checkmark$ & $\times$ & 11b & $\checkmark$ & $\checkmark$ & 16c & $\checkmark$ & $\checkmark$ & 24 & $\checkmark$ & $\checkmark$ & 28e & $\checkmark$ & ? & 35b & $\checkmark$ & $\times$ & 39b & $\checkmark$ & $\times$ & 44 & $\checkmark$ & $\checkmark$ & 49b & $\checkmark$ & $\times$ & 56 & $\checkmark$ & $\times$ & \textbf{Tot} & \textbf{85} & \textbf{[48, 54]} \\
% 6 & $\checkmark$ & $\checkmark$ & 11c & $\checkmark$ & $\checkmark$ & 17 & $\checkmark$ & $\times$ & 25 & $\checkmark$ & $\checkmark$ & 29 & $\checkmark$ & $\checkmark$ & 35c & $\checkmark$ & ? & 39c & $\checkmark$ & ? & 45a & $\checkmark$ & $\checkmark$ & 49c & $\checkmark$ & ? & 57 & $\checkmark$ & $\times$ &  &  &  \\
% 7 & $\checkmark$ & $\checkmark$ & 12 & $\checkmark$ & $\times$ & 18 & $\checkmark$ & $\checkmark$ & 26 & $\checkmark$ & $\times$ & 30 & $\checkmark$ & $\checkmark$ & 36a & $\checkmark$ & $\checkmark$ & 40 & $\checkmark$ & $\times$ & 45b & $\checkmark$ & $\checkmark$ & 50 & $\checkmark$ & $\checkmark$ & 58 & $\checkmark$ & $\checkmark$ &  &  &  \\

%         \bottomrule
%     \end{tabular}
% }
%     \label{tab:detect}
% \end{table*}

==> exp/tables/main_table.tex <==
\begin{table*}[!t]
\caption{Main evaluation results. \linyi{need to update with 10-seed results}}
    \centering
\resizebox{!}{0.44\textheight}{
\begin{tabular}{c|cc|cc|ccc|cc|cc|cc}
\toprule 
  &  & \# Defect  & \multicolumn{2}{c|}{System Test Generation (RQ1)} & \multicolumn{3}{c|}{Many Distinct Unit Test Generation (RQ2)} & \multicolumn{4}{c|}{Precondition-Fix Suggestion (RQ3)} & \multicolumn{2}{c}{Static Defect Detection (RQ4)} \\
  \cline{4-14}
  Case & \# & Nodes & \multicolumn{2}{c|}{\# Success among $D\times 10$ Trials $\uparrow$} & \multicolumn{3}{c|}{\# Success among $D\times 10 \times 1000$ Trials $\uparrow$~(Time $\downarrow$)} & \multicolumn{2}{c|}{Success for Weights + Input Nodes} & \multicolumn{2}{c|}{Success for Weights Nodes} & \multicolumn{2}{c}{Success Detection?} \\
  \cline{4-14}
  ID & Nodes & ($D$) & \textbf{\sysname} & Random & \textbf{\sysname} & Gradient Descent & Random & \textbf{\sysname} & Gradient Descent & \textbf{\sysname} & Gradient Descent & \textbf{\sysname} & DEBAR~\cite{zhang2020detecting} \\
\midrule 
1 & 181 & 1 & 0 (0.00) & 0 (0.00) & 1000 (153.23) & 1000 (86.93) & 305 (179.61) & $\checkmark$ (28.66) & $\times$ (180.31) & $\checkmark$ (27.79) & $\times$ (180.07) & $\checkmark$ & $\checkmark$ \\
2a & 18 & 2 & 2 (0.00) & 2 (0.01) & 2000 (0.55) & 2000 (0.44) & 1993 (14.07) & $\checkmark$ (0.32) & $\times$ (4.35) & $\checkmark$ (0.51) & $\times$ (3.81) & $\checkmark$ & $\checkmark$ \\
2b & 18 & 2 & 2 (0.00) & 2 (0.01) & 2000 (0.54) & 2000 (0.44) & 1989 (14.04) & $\checkmark$ (0.24) & $\times$ (4.24) & $\checkmark$ (0.43) & $\times$ (3.71) & $\checkmark$ & $\checkmark$ \\
3 & 12 & 1 & 1 (0.00) & 1 (0.01) & 1000 (0.20) & 1000 (0.13) & 1000 (3.91) & $\checkmark$ (0.18) & $\times$ (3.46) & $\checkmark$ (0.32) & $\times$ (2.90) & $\checkmark$ & $\checkmark$ \\
4 & 12 & 1 & 1 (0.00) & 1 (0.00) & 1000 (0.04) & 1000 (0.01) & 986 (1.16) & $\checkmark$ (0.09) & $\checkmark$ (0.06) & $\times$ (0.00) & $\times$ (0.00) & $\checkmark$ & $\times$ \\
5 & 43 & 1 & 1 (0.00) & 1 (0.01) & 1000 (0.80) & 1000 (0.29) & 111 (1.93) & $\checkmark$ (0.01) & $\checkmark$ (0.01) & $\times$ (0.00) & $\times$ (0.00) & $\checkmark$ & $\times$ \\
6 & 45 & 1 & 1 (0.00) & 1 (0.20) & 1000 (40.43) & 1000 (40.81) & 0 (0.00) & $\checkmark$ (1.64) & $\times$ (34.41) & $\checkmark$ (1.59) & $\times$ (31.47) & $\checkmark$ & $\checkmark$ \\
7 & 47 & 1 & 1 (0.00) & 1 (0.22) & 1000 (40.96) & 1000 (42.93) & 684 (179.82) & $\checkmark$ (1.68) & $\times$ (34.53) & $\checkmark$ (1.60) & $\times$ (31.75) & $\checkmark$ & $\checkmark$ \\
8 & 47 & 1 & 1 (0.00) & 1 (0.16) & 1000 (40.37) & 1000 (40.37) & 699 (179.69) & $\checkmark$ (1.91) & $\times$ (34.46) & $\checkmark$ (1.77) & $\times$ (31.59) & $\checkmark$ & $\checkmark$ \\
9a & 21 & 2 & 2 (0.00) & 2 (0.16) & 2000 (24.69) & 2000 (20.84) & 1574 (69.01) & $\checkmark$ (0.38) & $\times$ (4.93) & $\checkmark$ (0.36) & $\times$ (4.37) & $\checkmark$ & $\checkmark$ \\
9b & 21 & 2 & 2 (0.00) & 2 (0.18) & 2000 (24.27) & 2000 (20.33) & 1663 (67.07) & $\checkmark$ (0.30) & $\times$ (4.87) & $\checkmark$ (0.28) & $\times$ (4.29) & $\checkmark$ & $\checkmark$ \\
10 & 10 & 1 & 1 (0.09) & 1 (0.10) & 1000 (9.20) & 1000 (0.62) & 1000 (3.72) & $\checkmark$ (0.20) & $\times$ (3.09) & $\checkmark$ (0.29) & $\times$ (2.66) & $\checkmark$ & $\checkmark$ \\
11a & 27 & 1 & 1 (0.00) & 1 (0.02) & 1000 (3.45) & 1000 (3.26) & 999 (25.27) & $\checkmark$ (0.31) & $\checkmark$ (0.01) & $\checkmark$ (0.29) & $\checkmark$ (0.01) & $\checkmark$ & $\checkmark$ \\
11b & 29 & 1 & 1 (0.00) & 0 (0.00) & 1000 (8.01) & 1000 (7.01) & 997 (25.27) & $\checkmark$ (0.31) & $\checkmark$ (0.01) & $\checkmark$ (0.29) & $\checkmark$ (0.01) & $\checkmark$ & $\checkmark$ \\
11c & 21 & 1 & 1 (0.00) & 1 (0.02) & 1000 (3.45) & 1000 (3.39) & 998 (24.15) & $\checkmark$ (0.27) & $\checkmark$ (0.01) & $\checkmark$ (0.26) & $\checkmark$ (0.01) & $\checkmark$ & $\checkmark$ \\
12 & 14 & 1 & 1 (0.00) & 1 (0.09) & 1000 (13.69) & 1000 (7.10) & 1000 (46.68) & $\checkmark$ (0.35) & $\times$ (4.85) & $\checkmark$ (0.77) & $\times$ (4.40) & $\checkmark$ & $\times$ \\
13 & 15 & 1 & 1 (0.00) & 1 (0.00) & 1000 (0.03) & 1000 (0.01) & 981 (0.71) & $\checkmark$ (0.08) & $\checkmark$ (0.04) & $\times$ (0.00) & $\times$ (0.00) & $\checkmark$ & $\times$ \\
14 & 27 & 1 & 1 (0.17) & 1 (0.16) & 1000 (14.32) & 1000 (9.60) & 1000 (49.12) & $\checkmark$ (1.48) & $\times$ (30.79) & $\checkmark$ (1.66) & $\times$ (28.62) & $\checkmark$ & $\checkmark$ \\
15 & 96 & 1 & 0 (0.00) & 0 (0.00) & 1000 (24.75) & 0 (24.79) & 0 (48.47) & $\checkmark$ (7.64) & $\times$ (117.25) & $\checkmark$ (8.51) & $\times$ (117.67) & $\checkmark$ & $\checkmark$ \\
16a & 31 & 1 & 1 (0.00) & 1 (0.02) & 1000 (3.43) & 1000 (3.26) & 997 (24.73) & $\checkmark$ (0.39) & $\checkmark$ (0.03) & $\checkmark$ (0.37) & $\checkmark$ (0.03) & $\checkmark$ & $\checkmark$ \\
16b & 26 & 1 & 1 (0.00) & 0 (0.00) & 1000 (7.52) & 1000 (5.91) & 0 (23.76) & $\checkmark$ (0.31) & $\checkmark$ (0.03) & $\checkmark$ (0.30) & $\checkmark$ (0.02) & $\checkmark$ & $\checkmark$ \\
16c & 28 & 1 & 1 (0.00) & 0 (0.00) & 1000 (7.40) & 1000 (6.98) & 1 (23.53) & $\checkmark$ (0.31) & $\checkmark$ (0.02) & $\checkmark$ (0.29) & $\checkmark$ (0.02) & $\checkmark$ & $\checkmark$ \\
17 & 419 & 1 & 1 (111.15) & 1 (111.92) & 0 (180.00) & 0 (180.00) & 0 (0.00) & $\checkmark$ (12.33) & $\checkmark$ (0.52) & $\checkmark$ (12.34) & $\checkmark$ (0.49) & $\checkmark$ & $\times$ \\
18 & 15 & 1 & 1 (0.00) & 1 (0.01) & 1000 (0.22) & 1000 (0.14) & 1000 (3.89) & $\checkmark$ (0.26) & $\times$ (3.51) & $\checkmark$ (0.39) & $\times$ (3.01) & $\checkmark$ & $\checkmark$ \\
19 & 14 & 1 & 1 (0.09) & 1 (0.09) & 1000 (9.32) & 1000 (0.61) & 1000 (3.76) & $\checkmark$ (0.14) & $\times$ (3.14) & $\checkmark$ (0.25) & $\times$ (2.60) & $\checkmark$ & $\checkmark$ \\
20 & 13 & 1 & 1 (0.09) & 1 (0.09) & 1000 (9.38) & 1000 (0.67) & 1000 (3.69) & $\checkmark$ (0.14) & $\times$ (3.10) & $\checkmark$ (0.24) & $\times$ (2.60) & $\checkmark$ & $\checkmark$ \\
21 & 11 & 1 & 1 (0.08) & 1 (0.08) & 1000 (9.42) & 1000 (0.68) & 1000 (3.68) & $\checkmark$ (0.14) & $\times$ (3.09) & $\checkmark$ (0.24) & $\times$ (2.58) & $\checkmark$ & $\checkmark$ \\
22 & 28 & 2 & 2 (9.54) & 0 (0.00) & 2000 (43.46) & 2000 (52.97) & 2000 (163.53) & $\checkmark$ (0.25) & $\checkmark$ (0.25) & $\checkmark$ (0.43) & $\checkmark$ (0.42) & $\checkmark$ & $\times$ \\
23 & 15 & 1 & 1 (0.00) & 1 (0.00) & 1000 (0.05) & 1000 (0.01) & 419 (0.73) & $\checkmark$ (0.01) & $\checkmark$ (0.01) & $\times$ (0.00) & $\times$ (0.00) & $\checkmark$ & $\times$ \\
24 & 33 & 1 & 1 (0.00) & 1 (0.19) & 1000 (40.43) & 1000 (40.00) & 713 (179.91) & $\checkmark$ (1.52) & $\times$ (30.58) & $\checkmark$ (1.41) & $\times$ (27.91) & $\checkmark$ & $\checkmark$ \\
25 & 15 & 1 & 1 (0.00) & 1 (0.09) & 1000 (0.90) & 1000 (0.26) & 998 (4.00) & $\checkmark$ (0.27) & $\times$ (3.50) & $\checkmark$ (0.40) & $\times$ (3.00) & $\checkmark$ & $\checkmark$ \\
26 & 20 & 2 & 2 (0.03) & 2 (0.03) & 2000 (1.03) & 2000 (1.01) & 1838 (6.64) & $\checkmark$ (0.08) & $\times$ (3.86) & $\checkmark$ (0.14) & $\times$ (3.38) & $\checkmark$ & $\times$ \\
27 & 17 & 1 & 1 (0.00) & 1 (0.01) & 1000 (0.04) & 1000 (0.01) & 409 (0.71) & $\checkmark$ (0.01) & $\checkmark$ (0.01) & $\times$ (0.00) & $\times$ (0.00) & $\checkmark$ & $\times$ \\
28a & 89 & 1 & 1 (0.00) & 1 (0.03) & 1000 (2.45) & 1000 (2.17) & 1000 (29.83) & $\checkmark$ (0.34) & $\checkmark$ (0.19) & $\checkmark$ (0.34) & $\checkmark$ (0.19) & $\checkmark$ & $\checkmark$ \\
28b & 89 & 1 & 1 (0.00) & 1 (0.03) & 1000 (2.50) & 1000 (2.24) & 1000 (29.80) & $\checkmark$ (0.34) & $\checkmark$ (0.19) & $\checkmark$ (0.34) & $\checkmark$ (0.18) & $\checkmark$ & $\checkmark$ \\
28c & 91 & 3 & 0 (0.00) & 0 (0.00) & 0 (5.46) & 0 (12.50) & 0 (108.74) & $\checkmark$ (0.51) & $\checkmark$ (0.19) & $\checkmark$ (0.50) & $\checkmark$ (0.18) & $\checkmark$ & $\checkmark$ \\
28d & 89 & 2 & 0 (0.00) & 0 (0.00) & 0 (3.66) & 0 (6.80) & 0 (58.96) & $\checkmark$ (0.51) & $\checkmark$ (0.14) & $\checkmark$ (0.50) & $\checkmark$ (0.14) & $\checkmark$ & $\checkmark$ \\
28e & 91 & 2 & 0 (0.00) & 0 (0.00) & 0 (4.05) & 0 (6.65) & 0 (55.58) & $\checkmark$ (0.51) & $\checkmark$ (0.15) & $\checkmark$ (0.52) & $\checkmark$ (0.15) & $\checkmark$ & ? \\
29 & 47 & 1 & 1 (0.00) & 1 (0.20) & 1000 (40.93) & 1000 (40.56) & 679 (180.00) & $\checkmark$ (1.68) & $\times$ (34.96) & $\checkmark$ (1.60) & $\times$ (32.04) & $\checkmark$ & $\checkmark$ \\
30 & 12 & 1 & 1 (0.09) & 1 (0.09) & 1000 (9.18) & 1000 (0.63) & 1000 (3.69) & $\checkmark$ (0.14) & $\times$ (3.08) & $\checkmark$ (0.24) & $\times$ (2.55) & $\checkmark$ & $\checkmark$ \\
31 & 100 & 2 & 1 (0.15) & 1 (0.16) & 2000 (256.25) & 0 (141.46) & 206 (179.66) & $\checkmark$ (1.23) & $\times$ (25.06) & $\checkmark$ (1.22) & $\times$ (23.19) & $\checkmark$ & $\checkmark$ \\
32 & 19 & 1 & 1 (0.01) & 1 (0.01) & 1000 (0.94) & 1000 (0.44) & 1000 (1.90) & $\checkmark$ (0.07) & $\times$ (3.34) & $\checkmark$ (0.13) & $\times$ (2.88) & $\checkmark$ & $\times$ \\
33 & 18 & 2 & 2 (0.03) & 2 (0.03) & 2000 (0.98) & 2000 (0.97) & 1841 (6.37) & $\checkmark$ (0.08) & $\times$ (3.78) & $\checkmark$ (0.13) & $\times$ (3.27) & $\checkmark$ & $\times$ \\
34 & 21 & 1 & 1 (0.02) & 1 (0.02) & 1000 (0.81) & 1000 (0.35) & 1000 (1.93) & $\checkmark$ (0.07) & $\times$ (3.32) & $\checkmark$ (0.13) & $\times$ (2.83) & $\checkmark$ & $\times$ \\
35a & 52 & 1 & 1 (0.00) & 1 (0.53) & 1000 (26.88) & 1000 (21.90) & 1000 (49.01) & $\checkmark$ (0.33) & $\checkmark$ (0.01) & $\checkmark$ (0.32) & $\checkmark$ (0.01) & $\checkmark$ & $\checkmark$ \\
35b & 55 & 1 & 1 (0.00) & 1 (0.59) & 1000 (26.17) & 1000 (25.64) & 1000 (49.76) & $\checkmark$ (0.37) & $\times$ (7.57) & $\checkmark$ (0.35) & $\times$ (6.82) & $\checkmark$ & $\times$ \\
35c & 52 & 1 & 1 (0.00) & 1 (0.44) & 1000 (25.96) & 1000 (25.53) & 1000 (49.68) & $\checkmark$ (0.37) & $\times$ (7.51) & $\checkmark$ (0.36) & $\times$ (6.83) & $\checkmark$ & ? \\
36a & 53 & 1 & 1 (0.00) & 0 (0.00) & 1000 (25.71) & 1000 (24.58) & 701 (47.42) & $\checkmark$ (0.36) & $\times$ (7.43) & $\checkmark$ (0.35) & $\times$ (6.69) & $\checkmark$ & $\checkmark$ \\
36b & 49 & 1 & 1 (0.00) & 1 (0.34) & 1000 (26.30) & 1000 (21.24) & 679 (47.19) & $\checkmark$ (0.34) & $\checkmark$ (0.01) & $\checkmark$ (0.32) & $\checkmark$ (0.01) & $\checkmark$ & $\times$ \\
36c & 55 & 1 & 1 (0.35) & 1 (0.48) & 1000 (25.62) & 0 (15.53) & 711 (48.08) & $\checkmark$ (0.37) & $\times$ (7.51) & $\checkmark$ (0.36) & $\times$ (6.82) & $\checkmark$ & ? \\
37 & 17 & 2 & 1 (0.01) & 1 (0.01) & 2000 (1.69) & 2000 (0.77) & 293 (3.59) & $\checkmark$ (0.11) & $\times$ (3.72) & $\checkmark$ (0.19) & $\times$ (3.24) & $\checkmark$ & $\times$ \\
38 & 17 & 2 & 1 (0.01) & 1 (0.01) & 2000 (1.62) & 2000 (0.66) & 221 (3.54) & $\checkmark$ (0.10) & $\times$ (3.72) & $\checkmark$ (0.19) & $\times$ (3.26) & $\checkmark$ & $\times$ \\
39a & 53 & 1 & 0 (0.00) & 0 (0.00) & 1000 (36.22) & 0 (15.34) & 687 (47.72) & $\checkmark$ (0.37) & $\times$ (7.42) & $\checkmark$ (0.35) & $\times$ (6.68) & $\checkmark$ & $\checkmark$ \\
39b & 48 & 1 & 1 (0.00) & 0 (0.00) & 1000 (26.04) & 1000 (21.89) & 709 (50.81) & $\checkmark$ (0.32) & $\checkmark$ (0.01) & $\checkmark$ (0.31) & $\checkmark$ (0.01) & $\checkmark$ & $\times$ \\
39c & 55 & 1 & 1 (0.34) & 1 (0.38) & 1000 (36.83) & 0 (15.31) & 686 (49.74) & $\checkmark$ (0.37) & $\times$ (7.54) & $\checkmark$ (0.36) & $\times$ (6.81) & $\checkmark$ & ? \\
40 & 9 & 1 & 1 (0.01) & 1 (0.01) & 1000 (0.37) & 1000 (0.44) & 925 (1.31) & $\checkmark$ (0.06) & $\times$ (2.99) & $\checkmark$ (0.09) & $\times$ (2.44) & $\checkmark$ & $\times$ \\
41 & 11 & 1 & 1 (0.01) & 1 (0.01) & 1000 (0.36) & 1000 (0.37) & 920 (1.33) & $\checkmark$ (0.06) & $\times$ (3.08) & $\checkmark$ (0.10) & $\times$ (2.55) & $\checkmark$ & $\times$ \\
42 & 11 & 1 & 1 (0.01) & 1 (0.01) & 1000 (0.36) & 1000 (0.37) & 941 (1.39) & $\checkmark$ (0.06) & $\times$ (3.11) & $\checkmark$ (0.10) & $\times$ (2.56) & $\checkmark$ & $\times$ \\
43a & 56 & 1 & 1 (0.00) & 0 (0.00) & 1000 (25.45) & 1000 (25.11) & 700 (48.90) & $\checkmark$ (0.38) & $\times$ (7.84) & $\checkmark$ (0.37) & $\times$ (6.96) & $\checkmark$ & $\checkmark$ \\
43b & 51 & 1 & 1 (0.00) & 1 (0.37) & 1000 (26.54) & 1000 (22.85) & 676 (48.62) & $\checkmark$ (0.35) & $\checkmark$ (0.02) & $\checkmark$ (0.35) & $\checkmark$ (0.01) & $\checkmark$ & $\times$ \\
43c & 58 & 1 & 1 (0.00) & 0 (0.00) & 1000 (25.27) & 1000 (24.97) & 677 (49.52) & $\checkmark$ (0.39) & $\times$ (7.97) & $\checkmark$ (0.37) & $\times$ (7.06) & $\checkmark$ & ? \\
44 & 42 & 1 & 1 (0.00) & 1 (0.06) & 1000 (6.54) & 1000 (5.97) & 1000 (101.92) & $\checkmark$ (1.30) & $\times$ (26.70) & $\checkmark$ (1.34) & $\times$ (23.99) & $\checkmark$ & $\checkmark$ \\
45a & 13 & 1 & 1 (0.09) & 1 (0.09) & 1000 (9.23) & 1000 (0.68) & 1000 (3.67) & $\checkmark$ (0.23) & $\times$ (3.17) & $\checkmark$ (0.32) & $\times$ (2.64) & $\checkmark$ & $\checkmark$ \\
45b & 49 & 1 & 1 (0.00) & 1 (0.24) & 1000 (40.24) & 1000 (40.05) & 0 (0.00) & $\checkmark$ (1.68) & $\times$ (34.79) & $\checkmark$ (1.59) & $\times$ (31.63) & $\checkmark$ & $\checkmark$ \\
46 & 15 & 1 & 1 (0.00) & 1 (0.00) & 1000 (0.05) & 1000 (0.01) & 435 (0.63) & $\checkmark$ (0.01) & $\checkmark$ (0.01) & $\times$ (0.00) & $\times$ (0.00) & $\checkmark$ & $\times$ \\
47 & 20 & 1 & 1 (0.01) & 1 (0.02) & 1000 (0.87) & 1000 (0.36) & 1000 (1.90) & $\checkmark$ (0.15) & $\times$ (3.39) & $\checkmark$ (0.20) & $\times$ (2.90) & $\checkmark$ & $\times$ \\
48a & 34 & 1 & 1 (0.12) & 1 (0.08) & 1000 (10.31) & 0 (9.21) & 1000 (23.58) & $\checkmark$ (0.61) & $\times$ (6.86) & $\checkmark$ (1.05) & $\times$ (6.45) & $\checkmark$ & $\checkmark$ \\
48b & 13 & 1 & 1 (0.10) & 1 (0.08) & 1000 (9.16) & 1000 (0.69) & 1000 (3.66) & $\checkmark$ (0.14) & $\times$ (3.16) & $\checkmark$ (0.24) & $\times$ (2.55) & $\checkmark$ & $\checkmark$ \\
49a & 56 & 1 & 1 (0.00) & 0 (0.00) & 1000 (28.08) & 0 (15.64) & 692 (49.36) & $\checkmark$ (0.38) & $\times$ (8.10) & $\checkmark$ (0.36) & $\times$ (6.97) & $\checkmark$ & $\checkmark$ \\
49b & 51 & 1 & 1 (0.00) & 0 (0.00) & 1000 (27.83) & 1000 (22.54) & 674 (48.77) & $\checkmark$ (0.35) & $\checkmark$ (0.02) & $\checkmark$ (0.33) & $\checkmark$ (0.01) & $\checkmark$ & $\times$ \\
49c & 58 & 1 & 1 (0.52) & 1 (0.44) & 1000 (37.80) & 0 (16.06) & 710 (49.58) & $\checkmark$ (0.39) & $\times$ (8.29) & $\checkmark$ (0.37) & $\times$ (7.12) & $\checkmark$ & ? \\
50 & 13 & 1 & 1 (0.09) & 1 (0.08) & 1000 (9.40) & 1000 (0.62) & 1000 (3.65) & $\checkmark$ (0.14) & $\times$ (3.16) & $\checkmark$ (0.24) & $\times$ (2.55) & $\checkmark$ & $\checkmark$ \\
51 & 65 & 2 & 1 (0.57) & 1 (0.49) & 2000 (76.28) & 2000 (65.15) & 1000 (114.66) & $\checkmark$ (0.54) & $\times$ (11.39) & $\checkmark$ (1.08) & $\times$ (10.04) & $\checkmark$ & $\times$ \\
52 & 12 & 1 & 1 (0.09) & 1 (0.09) & 1000 (9.15) & 1000 (0.68) & 1000 (3.70) & $\checkmark$ (0.14) & $\times$ (3.15) & $\checkmark$ (0.24) & $\times$ (2.56) & $\checkmark$ & $\checkmark$ \\
53 & 17 & 2 & 2 (0.03) & 2 (0.03) & 2000 (1.40) & 2000 (0.90) & 1696 (7.12) & $\checkmark$ (0.07) & $\times$ (4.00) & $\checkmark$ (0.11) & $\times$ (3.35) & $\checkmark$ & $\times$ \\
54 & 12 & 1 & 1 (0.01) & 1 (0.01) & 1000 (0.81) & 1000 (0.34) & 1000 (1.92) & $\checkmark$ (0.07) & $\times$ (3.30) & $\checkmark$ (0.13) & $\times$ (2.76) & $\checkmark$ & $\times$ \\
55 & 49 & 1 & 1 (0.00) & 1 (0.18) & 1000 (41.08) & 1000 (38.80) & 669 (179.88) & $\checkmark$ (1.67) & $\times$ (34.85) & $\checkmark$ (1.61) & $\times$ (31.65) & $\checkmark$ & $\checkmark$ \\
56 & 20 & 2 & 2 (0.03) & 2 (0.03) & 2000 (1.05) & 2000 (0.99) & 1850 (6.79) & $\checkmark$ (0.17) & $\times$ (3.96) & $\checkmark$ (0.22) & $\times$ (3.48) & $\checkmark$ & $\times$ \\
57 & 19 & 1 & 1 (0.00) & 1 (0.00) & 1000 (0.04) & 1000 (0.01) & 404 (0.71) & $\checkmark$ (0.01) & $\checkmark$ (0.01) & $\times$ (0.00) & $\times$ (0.00) & $\checkmark$ & $\times$ \\
58 & 47 & 1 & 1 (0.00) & 1 (0.16) & 1000 (40.53) & 1000 (40.03) & 0 (0.00) & $\checkmark$ (1.68) & $\times$ (34.43) & $\checkmark$ (1.60) & $\times$ (31.81) & $\checkmark$ & $\checkmark$ \\
59 & 13 & 1 & 1 (0.00) & 1 (0.00) & 1000 (0.20) & 1000 (0.13) & 1000 (3.68) & $\checkmark$ (0.25) & $\times$ (3.16) & $\checkmark$ (0.36) & $\times$ (2.65) & $\checkmark$ & $\checkmark$ \\
60 & 11 & 1 & 1 (0.09) & 1 (0.09) & 1000 (9.37) & 1000 (0.61) & 1000 (3.69) & $\checkmark$ (0.23) & $\times$ (3.16) & $\checkmark$ (0.32) & $\times$ (2.64) & $\checkmark$ & $\checkmark$ \\
61 & 28 & 1 & 1 (0.12) & 1 (0.07) & 1000 (10.04) & 0 (8.16) & 1000 (19.84) & $\checkmark$ (0.48) & $\times$ (6.24) & $\checkmark$ (0.91) & $\times$ (5.60) & $\checkmark$ & $\checkmark$ \\
62 & 66 & 2 & 2 (19.30) & 1 (0.59) & 2000 (75.80) & 2000 (63.61) & 1000 (115.00) & $\checkmark$ (0.54) & $\times$ (11.06) & $\checkmark$ (1.07) & $\times$ (10.09) & $\checkmark$ & $\times$ \\
63 & 66 & 2 & 1 (0.47) & 1 (0.53) & 2000 (75.97) & 2000 (64.65) & 1000 (114.82) & $\checkmark$ (0.54) & $\times$ (11.06) & $\checkmark$ (1.07) & $\times$ (10.06) & $\checkmark$ & $\times$ \\
\midrule
\textbf{Tot} 85 & & 104 & 89 (143.94) & 77 (121.01) & 96000 (1901.39) & 86000 (1474.98) & 70736 (3488.78) & 85 (84.18) & 25 (892.59) & 78 (88.82) & 18 (833.32) & 85 & 48 - 54  \\
\bottomrule 
\end{tabular}
}

\label{tab:main}
\vspace{-1em}
\end{table*}


==> exp/tables/precond_table.tex <==
\begin{table*}[th]
    \centering
    \caption{(RQ3) Detail Results for precondition-fix suggestion for different imposing location requirements for \sysname and GD (baseline approach). ``$\checkmark$'' means precondition that fixes all numerical defects is found and ``$\times$'' means otherwise. ``Time (s)'' is the running time. 
    All approaches are deterministic.}
\resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccc|cccc||c|cccc|cccc||c|cccc|cccc}
        \toprule
        \multirow{2}{*}{Case} & \multicolumn{4}{c|}{Impose on Weight + Input} & \multicolumn{4}{c||}{Impose on Weight} &
        \multirow{2}{*}{Case} & \multicolumn{4}{c|}{Impose on Weight + Input} & \multicolumn{4}{c||}{Impose on Weight} &
        \multirow{2}{*}{Case} & \multicolumn{4}{c|}{Impose on Weight + Input} & \multicolumn{4}{c}{Impose on Weight} \\
        \cline{2-9}
        \cline{11-18}
        \cline{20-27}
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c|}{GD} & 
        \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c||}{GD} & 
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c|}{GD} & 
        \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c||}{GD} & 
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c|}{GD} & 
        \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GD} \\
        \cline{2-9}
        \cline{11-18}
        \cline{20-27}
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) \\
        % ID & $\checkmark$/$\times$ & Time & 
        % $\checkmark$/$\times$ & Time &
        % $\checkmark$/$\times$ & Time &
        % $\checkmark$/$\times$ & Time &
        % ID & $\checkmark$/$\times$ & Time & 
        % $\checkmark$/$\times$ & Time &
        % $\checkmark$/$\times$ & Time &
        % $\checkmark$/$\times$ & Time &
        % ID & $\checkmark$/$\times$ & Time & 
        % $\checkmark$/$\times$ & Time &
        % $\checkmark$/$\times$ & Time &
        % $\checkmark$/$\times$ & Time \\
        % & & (s) & & (s) & & (s) & & (s) & & (s) & & (s) 
        % & & (s) & & (s) & & (s) & & (s) & & (s) & & (s)  \\
        
        \hline

1 & $\checkmark$ & 19.91 & $\checkmark$ & 1.03 & $\checkmark$ & 20.30 & $\checkmark$ & 1.10 & 24 & $\checkmark$ & 1.12 & $\checkmark$ & 0.09 & $\checkmark$ & 0.88 & $\checkmark$ & 0.08 & 43a & $\checkmark$ & 0.13 & $\times$ & 7.71 & $\checkmark$ & 0.12 & $\times$ & 7.13 \\
2a & $\checkmark$ & 0.30 & $\checkmark$ & 0.41 & $\times$ & 3.54 & $\times$ & 3.97 & 25 & $\checkmark$ & 0.16 & $\checkmark$ & 0.25 & $\checkmark$ & 0.20 & $\times$ & 3.05 & 43b & $\checkmark$ & 0.12 & $\checkmark$ & 0.02 & $\checkmark$ & 0.11 & $\checkmark$ & 0.01 \\
2b & $\checkmark$ & 0.23 & $\checkmark$ & 0.23 & $\checkmark$ & 0.40 & $\times$ & 3.86 & 26 & $\checkmark$ & 0.08 & $\times$ & 3.87 & $\checkmark$ & 0.14 & $\times$ & 3.46 & 43c & $\checkmark$ & 0.13 & $\times$ & 7.80 & $\checkmark$ & 0.12 & $\times$ & 7.23 \\
3 & $\checkmark$ & 0.13 & $\checkmark$ & 0.23 & $\checkmark$ & 0.23 & $\times$ & 2.95 & 27 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 & 44 & $\checkmark$ & 0.71 & $\checkmark$ & 0.07 & $\checkmark$ & 0.65 & $\checkmark$ & 0.07 \\
4 & $\checkmark$ & 0.10 & $\checkmark$ & 0.06 & $\times$ & 0.00 & $\times$ & 0.00 & 28a & $\checkmark$ & 0.92 & $\times$ & 17.11 & $\checkmark$ & 1.20 & $\times$ & 16.89 & 45a & $\checkmark$ & 0.24 & $\checkmark$ & 0.24 & $\checkmark$ & 0.34 & $\checkmark$ & 0.34 \\
5 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 & 28b & $\checkmark$ & 0.90 & $\times$ & 17.62 & $\checkmark$ & 1.20 & $\times$ & 16.79 & 45b & $\checkmark$ & 1.28 & $\checkmark$ & 0.10 & $\checkmark$ & 1.16 & $\checkmark$ & 0.09 \\
6 & $\checkmark$ & 1.21 & $\checkmark$ & 0.09 & $\checkmark$ & 1.19 & $\checkmark$ & 0.09 & 28c & $\checkmark$ & 0.31 & $\checkmark$ & 0.07 & $\checkmark$ & 0.31 & $\checkmark$ & 0.07 & 46 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 \\
7 & $\checkmark$ & 1.27 & $\checkmark$ & 0.14 & $\checkmark$ & 1.18 & $\checkmark$ & 0.09 & 28d & $\checkmark$ & 0.05 & $\checkmark$ & 0.02 & $\checkmark$ & 0.05 & $\checkmark$ & 0.02 & 47 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.21 & $\checkmark$ & 0.21 \\
8 & $\checkmark$ & 1.36 & $\checkmark$ & 0.10 & $\checkmark$ & 1.20 & $\checkmark$ & 0.09 & 28e & $\checkmark$ & 0.05 & $\checkmark$ & 0.02 & $\checkmark$ & 0.05 & $\checkmark$ & 0.02 & 48a & $\checkmark$ & 0.33 & $\checkmark$ & 0.80 & $\checkmark$ & 0.51 & $\checkmark$ & 0.50 \\
9a & $\checkmark$ & 0.34 & $\times$ & 4.85 & $\checkmark$ & 0.31 & $\times$ & 4.45 & 29 & $\checkmark$ & 1.13 & $\checkmark$ & 0.10 & $\checkmark$ & 1.04 & $\checkmark$ & 0.09 & 48b & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 \\
9b & $\checkmark$ & 0.25 & $\times$ & 4.78 & $\checkmark$ & 0.23 & $\times$ & 4.40 & 30 & $\checkmark$ & 0.15 & $\checkmark$ & 0.16 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & 49a & $\checkmark$ & 0.13 & $\times$ & 7.71 & $\checkmark$ & 0.12 & $\times$ & 7.12 \\
10 & $\checkmark$ & 0.22 & $\checkmark$ & 0.22 & $\checkmark$ & 0.32 & $\checkmark$ & 0.33 & 31 & $\checkmark$ & 0.22 & $\times$ & 25.30 & $\checkmark$ & 0.22 & $\times$ & 23.72 & 49b & $\checkmark$ & 0.12 & $\checkmark$ & 0.02 & $\checkmark$ & 0.11 & $\checkmark$ & 0.01 \\
11a & $\checkmark$ & 0.17 & $\checkmark$ & 0.01 & $\checkmark$ & 0.16 & $\checkmark$ & 0.01 & 32 & $\checkmark$ & 0.08 & $\checkmark$ & 0.08 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & 49c & $\checkmark$ & 0.13 & $\times$ & 7.79 & $\checkmark$ & 0.12 & $\times$ & 7.24 \\
11b & $\checkmark$ & 0.17 & $\checkmark$ & 0.01 & $\checkmark$ & 0.16 & $\checkmark$ & 0.01 & 33 & $\checkmark$ & 0.08 & $\times$ & 3.76 & $\checkmark$ & 0.13 & $\times$ & 3.34 & 50 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 \\
11c & $\checkmark$ & 0.15 & $\checkmark$ & 0.01 & $\checkmark$ & 0.14 & $\checkmark$ & 0.01 & 34 & $\checkmark$ & 0.08 & $\checkmark$ & 0.08 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & 51 & $\checkmark$ & 0.16 & $\checkmark$ & 0.78 & $\checkmark$ & 0.30 & $\times$ & 10.13 \\
12 & $\checkmark$ & 0.10 & $\checkmark$ & 0.15 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & 35a & $\checkmark$ & 0.11 & $\checkmark$ & 0.01 & $\checkmark$ & 0.10 & $\checkmark$ & 0.01 & 52 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 \\
13 & $\checkmark$ & 0.08 & $\checkmark$ & 0.05 & $\times$ & 0.00 & $\times$ & 0.00 & 35b & $\checkmark$ & 0.12 & $\times$ & 7.36 & $\checkmark$ & 0.11 & $\times$ & 6.94 & 53 & $\checkmark$ & 0.07 & $\times$ & 3.83 & $\checkmark$ & 0.12 & $\times$ & 3.44 \\
14 & $\checkmark$ & 0.76 & $\checkmark$ & 0.05 & $\checkmark$ & 0.77 & $\checkmark$ & 0.05 & 35c & $\checkmark$ & 0.12 & $\times$ & 7.39 & $\checkmark$ & 0.12 & $\times$ & 6.93 & 54 & $\checkmark$ & 0.07 & $\checkmark$ & 0.07 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 \\
15 & $\checkmark$ & 0.19 & $\checkmark$ & 0.20 & $\checkmark$ & 0.19 & $\checkmark$ & 0.19 & 36a & $\checkmark$ & 0.12 & $\times$ & 7.24 & $\checkmark$ & 0.11 & $\times$ & 6.85 & 55 & $\checkmark$ & 1.22 & $\checkmark$ & 0.10 & $\checkmark$ & 1.31 & $\checkmark$ & 0.09 \\
16a & $\checkmark$ & 0.25 & $\checkmark$ & 0.03 & $\checkmark$ & 0.24 & $\checkmark$ & 0.03 & 36b & $\checkmark$ & 0.11 & $\checkmark$ & 0.02 & $\checkmark$ & 0.10 & $\checkmark$ & 0.01 & 56 & $\checkmark$ & 0.16 & $\times$ & 3.96 & $\checkmark$ & 0.22 & $\times$ & 3.58 \\
16b & $\checkmark$ & 0.17 & $\checkmark$ & 0.03 & $\checkmark$ & 0.16 & $\checkmark$ & 0.02 & 36c & $\checkmark$ & 0.12 & $\times$ & 7.35 & $\checkmark$ & 0.11 & $\times$ & 6.95 & 57 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 \\
16c & $\checkmark$ & 0.17 & $\checkmark$ & 0.02 & $\checkmark$ & 0.16 & $\checkmark$ & 0.02 & 37 & $\checkmark$ & 0.03 & $\times$ & 3.33 & $\checkmark$ & 0.05 & $\times$ & 2.94 & 58 & $\checkmark$ & 1.22 & $\checkmark$ & 0.10 & $\checkmark$ & 1.19 & $\checkmark$ & 0.11 \\
17 & $\checkmark$ & 3.41 & $\checkmark$ & 0.48 & $\checkmark$ & 3.54 & $\checkmark$ & 0.45 & 38 & $\checkmark$ & 0.03 & $\times$ & 3.31 & $\checkmark$ & 0.05 & $\times$ & 2.94 & 59 & $\checkmark$ & 0.22 & $\checkmark$ & 0.22 & $\checkmark$ & 0.30 & $\checkmark$ & 0.31 \\
18 & $\checkmark$ & 0.18 & $\checkmark$ & 0.18 & $\checkmark$ & 0.26 & $\checkmark$ & 0.26 & 39a & $\checkmark$ & 0.12 & $\times$ & 7.25 & $\checkmark$ & 0.11 & $\times$ & 6.86 & 60 & $\checkmark$ & 0.24 & $\checkmark$ & 0.23 & $\checkmark$ & 0.33 & $\checkmark$ & 0.34 \\
19 & $\checkmark$ & 0.14 & $\times$ & 3.09 & $\checkmark$ & 0.25 & $\times$ & 2.65 & 39b & $\checkmark$ & 0.11 & $\checkmark$ & 0.01 & $\checkmark$ & 0.10 & $\checkmark$ & 0.01 & 61 & $\checkmark$ & 0.30 & $\checkmark$ & 0.73 & $\checkmark$ & 0.45 & $\checkmark$ & 0.44 \\
20 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & 39c & $\checkmark$ & 0.12 & $\times$ & 7.37 & $\checkmark$ & 0.12 & $\times$ & 6.98 & 62 & $\checkmark$ & 0.18 & $\checkmark$ & 1.49 & $\checkmark$ & 0.32 & $\times$ & 10.15 \\
21 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & 40 & $\checkmark$ & 0.06 & $\checkmark$ & 0.06 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & 63 & $\checkmark$ & 0.17 & $\checkmark$ & 2.77 & $\checkmark$ & 0.30 & $\times$ & 10.16 \\
\cline{19-27}
22 & $\checkmark$ & 0.08 & $\checkmark$ & 0.14 & $\checkmark$ & 0.13 & $\checkmark$ & 0.12 & 41 & $\checkmark$ & 0.06 & $\checkmark$ & 0.06 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & \textbf{Tot} & \textbf{85} & \textbf{46.26} & \textbf{63} & \textbf{183.42} & \textbf{77} & \textbf{52.27} & \textbf{49} & \textbf{211.19} \\
23 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 & 42 & $\checkmark$ & 0.06 & $\checkmark$ & 0.06 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 &  &  &  &  &  &  &  &  &  \\


        \bottomrule
    \end{tabular}
}
    \label{tab:precond}
\end{table*}


% \begin{table*}[th]
%     \centering
%     \caption{Statistics for precondition-fix suggestion.}
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{ccccccccccccc|ccccccccccccc|ccccccccccccc}
%         \toprule
%         & \multicolumn{4}{c}{Impose on Weight + Input} & \multicolumn{4}{c}{Impose on Weight} & \multicolumn{4}{c|}{Impose on Input} &
%         & \multicolumn{4}{c}{Impose on Weight + Input} & \multicolumn{4}{c}{Impose on Weight} & \multicolumn{4}{c|}{Impose on Input} &
%         & \multicolumn{4}{c}{Impose on Weight + Input} & \multicolumn{4}{c}{Impose on Weight} & \multicolumn{4}{c}{Impose on Input} \\
%         Case & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GD} & 
%         \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GD} & 
%         \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c|}{GD} & Case & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GD} & 
%         \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GD} & 
%         \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c|}{GD} & Case & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GD} & 
%         \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GD} & 
%         \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GD} \\
%         ID & $\checkmark$/$\times$ & Time & 
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time & 
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time &
%         ID & $\checkmark$/$\times$ & Time & 
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time & 
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time &
%         ID & $\checkmark$/$\times$ & Time & 
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time & 
%         $\checkmark$/$\times$ & Time &
%         $\checkmark$/$\times$ & Time \\
%         & & (s) & & (s) & & (s) & & (s) & & (s) & & (s) 
%         & & (s) & & (s) & & (s) & & (s) & & (s) & & (s) 
%         & & (s) & & (s) & & (s) & & (s) & & (s) & & (s) \\
        
%         \hline

% 1 & $\checkmark$ & 19.91 & $\checkmark$ & 1.03 & $\checkmark$ & 20.30 & $\checkmark$ & 1.10 & $\times$ & 180.21 & $\times$ & 180.35 & 24 & $\checkmark$ & 1.12 & $\checkmark$ & 0.09 & $\checkmark$ & 0.88 & $\checkmark$ & 0.08 & $\times$ & 24.83 & $\times$ & 24.39 & 43a & $\checkmark$ & 0.13 & $\times$ & 7.71 & $\checkmark$ & 0.12 & $\times$ & 7.13 & $\times$ & 6.45 & $\times$ & 6.21 \\
% 2a & $\checkmark$ & 0.30 & $\checkmark$ & 0.41 & $\times$ & 3.54 & $\times$ & 3.97 & $\checkmark$ & 0.47 & $\checkmark$ & 0.46 & 25 & $\checkmark$ & 0.16 & $\checkmark$ & 0.25 & $\checkmark$ & 0.20 & $\times$ & 3.05 & $\checkmark$ & 0.19 & $\checkmark$ & 0.18 & 43b & $\checkmark$ & 0.12 & $\checkmark$ & 0.02 & $\checkmark$ & 0.11 & $\checkmark$ & 0.01 & $\times$ & 5.97 & $\times$ & 5.78 \\
% 2b & $\checkmark$ & 0.23 & $\checkmark$ & 0.23 & $\checkmark$ & 0.40 & $\times$ & 3.86 & $\checkmark$ & 0.38 & $\checkmark$ & 0.38 & 26 & $\checkmark$ & 0.08 & $\times$ & 3.87 & $\checkmark$ & 0.14 & $\times$ & 3.46 & $\checkmark$ & 0.14 & $\times$ & 3.16 & 43c & $\checkmark$ & 0.13 & $\times$ & 7.80 & $\checkmark$ & 0.12 & $\times$ & 7.23 & $\times$ & 6.54 & $\times$ & 6.31 \\
% 3 & $\checkmark$ & 0.13 & $\checkmark$ & 0.23 & $\checkmark$ & 0.23 & $\times$ & 2.95 & $\checkmark$ & 0.22 & $\checkmark$ & 0.22 & 27 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & 44 & $\checkmark$ & 0.71 & $\checkmark$ & 0.07 & $\checkmark$ & 0.65 & $\checkmark$ & 0.07 & $\times$ & 21.55 & $\times$ & 20.93 \\
% 4 & $\checkmark$ & 0.10 & $\checkmark$ & 0.06 & $\times$ & 0.00 & $\times$ & 0.00 & $\checkmark$ & 0.09 & $\checkmark$ & 0.05 & 28a & $\checkmark$ & 0.92 & $\times$ & 17.11 & $\checkmark$ & 1.20 & $\times$ & 16.89 & $\times$ & 12.81 & $\times$ & 12.64 & 45a & $\checkmark$ & 0.24 & $\checkmark$ & 0.24 & $\checkmark$ & 0.34 & $\checkmark$ & 0.34 & $\checkmark$ & 0.35 & $\checkmark$ & 0.34 \\
% 5 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & 28b & $\checkmark$ & 0.90 & $\times$ & 17.62 & $\checkmark$ & 1.20 & $\times$ & 16.79 & $\times$ & 12.81 & $\times$ & 12.65 & 45b & $\checkmark$ & 1.28 & $\checkmark$ & 0.10 & $\checkmark$ & 1.16 & $\checkmark$ & 0.09 & $\times$ & 28.17 & $\times$ & 27.20 \\
% 6 & $\checkmark$ & 1.21 & $\checkmark$ & 0.09 & $\checkmark$ & 1.19 & $\checkmark$ & 0.09 & $\times$ & 27.96 & $\times$ & 28.33 & 28c & $\checkmark$ & 0.31 & $\checkmark$ & 0.07 & $\checkmark$ & 0.31 & $\checkmark$ & 0.07 & $\times$ & 0.01 & $\times$ & 0.01 & 46 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 \\
% 7 & $\checkmark$ & 1.27 & $\checkmark$ & 0.14 & $\checkmark$ & 1.18 & $\checkmark$ & 0.09 & $\times$ & 28.12 & $\times$ & 27.75 & 28d & $\checkmark$ & 0.05 & $\checkmark$ & 0.02 & $\checkmark$ & 0.05 & $\checkmark$ & 0.02 & $\times$ & 0.01 & $\times$ & 0.01 & 47 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.21 & $\checkmark$ & 0.21 & $\checkmark$ & 0.20 & $\checkmark$ & 0.19 \\
% 8 & $\checkmark$ & 1.36 & $\checkmark$ & 0.10 & $\checkmark$ & 1.20 & $\checkmark$ & 0.09 & $\times$ & 28.23 & $\times$ & 27.73 & 28e & $\checkmark$ & 0.05 & $\checkmark$ & 0.02 & $\checkmark$ & 0.05 & $\checkmark$ & 0.02 & $\times$ & 0.01 & $\times$ & 0.01 & 48a & $\checkmark$ & 0.33 & $\checkmark$ & 0.80 & $\checkmark$ & 0.51 & $\checkmark$ & 0.50 & $\times$ & 5.48 & $\times$ & 5.37 \\
% 9a & $\checkmark$ & 0.34 & $\times$ & 4.85 & $\checkmark$ & 0.31 & $\times$ & 4.45 & $\times$ & 4.12 & $\times$ & 4.03 & 29 & $\checkmark$ & 1.13 & $\checkmark$ & 0.10 & $\checkmark$ & 1.04 & $\checkmark$ & 0.09 & $\times$ & 28.33 & $\times$ & 27.40 & 48b & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 \\
% 9b & $\checkmark$ & 0.25 & $\times$ & 4.78 & $\checkmark$ & 0.23 & $\times$ & 4.40 & $\times$ & 4.05 & $\times$ & 3.96 & 30 & $\checkmark$ & 0.15 & $\checkmark$ & 0.16 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & 49a & $\checkmark$ & 0.13 & $\times$ & 7.71 & $\checkmark$ & 0.12 & $\times$ & 7.12 & $\times$ & 6.41 & $\times$ & 6.21 \\
% 10 & $\checkmark$ & 0.22 & $\checkmark$ & 0.22 & $\checkmark$ & 0.32 & $\checkmark$ & 0.33 & $\checkmark$ & 0.31 & $\checkmark$ & 0.30 & 31 & $\checkmark$ & 0.22 & $\times$ & 25.30 & $\checkmark$ & 0.22 & $\times$ & 23.72 & $\times$ & 21.09 & $\times$ & 20.37 & 49b & $\checkmark$ & 0.12 & $\checkmark$ & 0.02 & $\checkmark$ & 0.11 & $\checkmark$ & 0.01 & $\times$ & 5.97 & $\times$ & 5.83 \\
% 11a & $\checkmark$ & 0.17 & $\checkmark$ & 0.01 & $\checkmark$ & 0.16 & $\checkmark$ & 0.01 & $\times$ & 5.14 & $\times$ & 4.92 & 32 & $\checkmark$ & 0.08 & $\checkmark$ & 0.08 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & 49c & $\checkmark$ & 0.13 & $\times$ & 7.79 & $\checkmark$ & 0.12 & $\times$ & 7.24 & $\times$ & 6.52 & $\times$ & 6.48 \\
% 11b & $\checkmark$ & 0.17 & $\checkmark$ & 0.01 & $\checkmark$ & 0.16 & $\checkmark$ & 0.01 & $\times$ & 5.13 & $\times$ & 4.93 & 33 & $\checkmark$ & 0.08 & $\times$ & 3.76 & $\checkmark$ & 0.13 & $\times$ & 3.34 & $\checkmark$ & 0.13 & $\times$ & 3.05 & 50 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 \\
% 11c & $\checkmark$ & 0.15 & $\checkmark$ & 0.01 & $\checkmark$ & 0.14 & $\checkmark$ & 0.01 & $\times$ & 4.46 & $\times$ & 4.31 & 34 & $\checkmark$ & 0.08 & $\checkmark$ & 0.08 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & 51 & $\checkmark$ & 0.16 & $\checkmark$ & 0.78 & $\checkmark$ & 0.30 & $\times$ & 10.13 & $\checkmark$ & 0.27 & $\checkmark$ & 0.25 \\
% 12 & $\checkmark$ & 0.10 & $\checkmark$ & 0.15 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & $\checkmark$ & 0.20 & $\checkmark$ & 0.19 & 35a & $\checkmark$ & 0.11 & $\checkmark$ & 0.01 & $\checkmark$ & 0.10 & $\checkmark$ & 0.01 & $\times$ & 5.49 & $\times$ & 5.38 & 52 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.26 \\
% 13 & $\checkmark$ & 0.08 & $\checkmark$ & 0.05 & $\times$ & 0.00 & $\times$ & 0.00 & $\checkmark$ & 0.07 & $\checkmark$ & 0.04 & 35b & $\checkmark$ & 0.12 & $\times$ & 7.36 & $\checkmark$ & 0.11 & $\times$ & 6.94 & $\times$ & 6.07 & $\times$ & 5.89 & 53 & $\checkmark$ & 0.07 & $\times$ & 3.83 & $\checkmark$ & 0.12 & $\times$ & 3.44 & $\checkmark$ & 0.11 & $\times$ & 3.24 \\
% 14 & $\checkmark$ & 0.76 & $\checkmark$ & 0.05 & $\checkmark$ & 0.77 & $\checkmark$ & 0.05 & $\times$ & 25.98 & $\times$ & 25.03 & 35c & $\checkmark$ & 0.12 & $\times$ & 7.39 & $\checkmark$ & 0.12 & $\times$ & 6.93 & $\times$ & 6.09 & $\times$ & 5.90 & 54 & $\checkmark$ & 0.07 & $\checkmark$ & 0.07 & $\checkmark$ & 0.13 & $\checkmark$ & 0.13 & $\checkmark$ & 0.12 & $\checkmark$ & 0.12 \\
% 15 & $\checkmark$ & 0.19 & $\checkmark$ & 0.20 & $\checkmark$ & 0.19 & $\checkmark$ & 0.19 & $\checkmark$ & 0.18 & $\checkmark$ & 0.18 & 36a & $\checkmark$ & 0.12 & $\times$ & 7.24 & $\checkmark$ & 0.11 & $\times$ & 6.85 & $\times$ & 5.98 & $\times$ & 5.79 & 55 & $\checkmark$ & 1.22 & $\checkmark$ & 0.10 & $\checkmark$ & 1.31 & $\checkmark$ & 0.09 & $\times$ & 28.04 & $\times$ & 28.78 \\
% 16a & $\checkmark$ & 0.25 & $\checkmark$ & 0.03 & $\checkmark$ & 0.24 & $\checkmark$ & 0.03 & $\times$ & 5.23 & $\times$ & 5.04 & 36b & $\checkmark$ & 0.11 & $\checkmark$ & 0.02 & $\checkmark$ & 0.10 & $\checkmark$ & 0.01 & $\times$ & 5.51 & $\times$ & 5.39 & 56 & $\checkmark$ & 0.16 & $\times$ & 3.96 & $\checkmark$ & 0.22 & $\times$ & 3.58 & $\checkmark$ & 0.22 & $\times$ & 3.34 \\
% 16b & $\checkmark$ & 0.17 & $\checkmark$ & 0.03 & $\checkmark$ & 0.16 & $\checkmark$ & 0.02 & $\times$ & 5.19 & $\times$ & 5.02 & 36c & $\checkmark$ & 0.12 & $\times$ & 7.35 & $\checkmark$ & 0.11 & $\times$ & 6.95 & $\times$ & 6.09 & $\times$ & 5.86 & 57 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 \\
% 16c & $\checkmark$ & 0.17 & $\checkmark$ & 0.02 & $\checkmark$ & 0.16 & $\checkmark$ & 0.02 & $\times$ & 5.19 & $\times$ & 5.03 & 37 & $\checkmark$ & 0.03 & $\times$ & 3.33 & $\checkmark$ & 0.05 & $\times$ & 2.94 & $\checkmark$ & 0.05 & $\times$ & 2.69 & 58 & $\checkmark$ & 1.22 & $\checkmark$ & 0.10 & $\checkmark$ & 1.19 & $\checkmark$ & 0.11 & $\times$ & 27.93 & $\times$ & 28.12 \\
% 17 & $\checkmark$ & 3.41 & $\checkmark$ & 0.48 & $\checkmark$ & 3.54 & $\checkmark$ & 0.45 & $\times$ & 180.03 & $\times$ & 180.15 & 38 & $\checkmark$ & 0.03 & $\times$ & 3.31 & $\checkmark$ & 0.05 & $\times$ & 2.94 & $\checkmark$ & 0.05 & $\times$ & 2.69 & 59 & $\checkmark$ & 0.22 & $\checkmark$ & 0.22 & $\checkmark$ & 0.30 & $\checkmark$ & 0.31 & $\checkmark$ & 0.32 & $\checkmark$ & 0.31 \\
% 18 & $\checkmark$ & 0.18 & $\checkmark$ & 0.18 & $\checkmark$ & 0.26 & $\checkmark$ & 0.26 & $\times$ & 2.99 & $\times$ & 2.91 & 39a & $\checkmark$ & 0.12 & $\times$ & 7.25 & $\checkmark$ & 0.11 & $\times$ & 6.86 & $\times$ & 5.98 & $\times$ & 5.77 & 60 & $\checkmark$ & 0.24 & $\checkmark$ & 0.23 & $\checkmark$ & 0.33 & $\checkmark$ & 0.34 & $\checkmark$ & 0.34 & $\checkmark$ & 0.33 \\
% 19 & $\checkmark$ & 0.14 & $\times$ & 3.09 & $\checkmark$ & 0.25 & $\times$ & 2.65 & $\checkmark$ & 0.25 & $\times$ & 2.65 & 39b & $\checkmark$ & 0.11 & $\checkmark$ & 0.01 & $\checkmark$ & 0.10 & $\checkmark$ & 0.01 & $\times$ & 5.38 & $\times$ & 5.28 & 61 & $\checkmark$ & 0.30 & $\checkmark$ & 0.73 & $\checkmark$ & 0.45 & $\checkmark$ & 0.44 & $\times$ & 5.19 & $\times$ & 5.07 \\
% 20 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & 39c & $\checkmark$ & 0.12 & $\times$ & 7.37 & $\checkmark$ & 0.12 & $\times$ & 6.98 & $\times$ & 6.07 & $\times$ & 5.89 & 62 & $\checkmark$ & 0.18 & $\checkmark$ & 1.49 & $\checkmark$ & 0.32 & $\times$ & 10.15 & $\checkmark$ & 0.30 & $\checkmark$ & 0.28 \\
% 21 & $\checkmark$ & 0.15 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.26 & $\checkmark$ & 0.25 & 40 & $\checkmark$ & 0.06 & $\checkmark$ & 0.06 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & 63 & $\checkmark$ & 0.17 & $\checkmark$ & 2.77 & $\checkmark$ & 0.30 & $\times$ & 10.16 & $\checkmark$ & 0.27 & $\checkmark$ & 0.26 \\
% \cline{27-39}
% 22 & $\checkmark$ & 0.08 & $\checkmark$ & 0.14 & $\checkmark$ & 0.13 & $\checkmark$ & 0.12 & $\checkmark$ & 0.12 & $\checkmark$ & 0.12 & 41 & $\checkmark$ & 0.06 & $\checkmark$ & 0.06 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & \textbf{Tot} & \textbf{85} & \textbf{46.26} & \textbf{63} & \textbf{183.42} & \textbf{77} & \textbf{52.27} & \textbf{49} & \textbf{211.19} & \textbf{41} & \textbf{826.26} & \textbf{34} & \textbf{837.55} \\
% 23 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\times$ & 0.00 & $\times$ & 0.00 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & 42 & $\checkmark$ & 0.06 & $\checkmark$ & 0.06 & $\checkmark$ & 0.10 & $\checkmark$ & 0.10 & $\checkmark$ & 0.11 & $\checkmark$ & 0.10 &  &  &  &  &  &  &  &  &  &  &  &  &  \\

%         \bottomrule
%     \end{tabular}
% }
%     \label{tab:precond}
% \end{table*}

==> exp/tables/precond_table_input.tex <==
\begin{table*}[th]
    \centering
    \caption{Detail Results for precondition-fix suggestion for  imposing on  \underline{only input nodes} for \sysname and baseline approaches~(\sysname-E and GD). ``$\checkmark$'' means precondition that fixes all numerical defects is found and ``$\times$'' means otherwise. ``Time (s)'' is the running time. 
    All approaches are deterministic.}
\resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|cccccc||c|cccccc||c|cccccc}
        \toprule
        \multirow{2}{*}{Case} & \multicolumn{6}{c|}{Impose on Input} & 
        \multirow{2}{*}{Case} & \multicolumn{6}{c|}{Impose on Input} &
        \multirow{2}{*}{Case} & \multicolumn{6}{c}{Impose on Input} \\
        \cline{2-7}
        \cline{9-14}
        \cline{16-21}
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c|}{GD} &
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c|}{GD} &
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c}{GD} \\
        \cline{2-7}
        \cline{9-14}
        \cline{16-21}
        
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s)  \\
        
        \hline

1 & $\times$ & 180.14 & $\times$ & 180.14 & $\times$ & 180.38 & 24 & $\times$ & 31.59 & $\times$ & 180.30 & $\times$ & 27.48 & 43a & $\times$ & 6.68 & $\times$ & 83.78 & $\times$ & 6.44 \\
2a & $\checkmark$ & 0.49 & $\checkmark$ & 0.74 & $\checkmark$ & 0.48 & 25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.36 & $\checkmark$ & 0.25 & 43b & $\times$ & 6.35 & $\times$ & 78.19 & $\times$ & 6.10 \\
2b & $\checkmark$ & 0.40 & $\checkmark$ & 0.68 & $\checkmark$ & 0.39 & 26 & $\checkmark$ & 0.14 & $\checkmark$ & 0.17 & $\times$ & 3.27 & 43c & $\times$ & 7.23 & $\times$ & 94.45 & $\times$ & 6.54 \\
3 & $\checkmark$ & 0.23 & $\checkmark$ & 0.42 & $\checkmark$ & 0.22 & 27 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & 44 & $\times$ & 27.51 & $\times$ & 178.82 & $\times$ & 22.94 \\
4 & $\checkmark$ & 0.09 & $\checkmark$ & 0.19 & $\checkmark$ & 0.06 & 28a & $\times$ & 13.99 & $\times$ & 65.12 & $\times$ & 13.03 & 45a & $\checkmark$ & 0.36 & $\checkmark$ & 0.55 & $\checkmark$ & 0.35 \\
5 & $\checkmark$ & 0.01 & $\checkmark$ & 0.04 & $\checkmark$ & 0.01 & 28b & $\times$ & 13.89 & $\times$ & 64.84 & $\times$ & 13.02 & 45b & $\times$ & 38.52 & $\times$ & 180.24 & $\times$ & 31.01 \\
6 & $\times$ & 37.51 & $\times$ & 180.25 & $\times$ & 30.81 & 28c & $\times$ & 0.01 & $\times$ & 0.07 & $\times$ & 0.01 & 46 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 \\
7 & $\times$ & 38.60 & $\times$ & 180.20 & $\times$ & 30.70 & 28d & $\times$ & 0.01 & $\times$ & 0.09 & $\times$ & 0.01 & 47 & $\checkmark$ & 0.22 & $\checkmark$ & 0.25 & $\checkmark$ & 0.20 \\
8 & $\times$ & 38.37 & $\times$ & 180.24 & $\times$ & 30.85 & 28e & $\times$ & 0.01 & $\times$ & 0.07 & $\times$ & 0.01 & 48a & $\times$ & 6.02 & $\times$ & 46.94 & $\times$ & 5.58 \\
9a & $\times$ & 4.39 & $\times$ & 45.41 & $\times$ & 4.10 & 29 & $\times$ & 46.05 & $\times$ & 180.13 & $\times$ & 30.77 & 48b & $\checkmark$ & 0.28 & $\checkmark$ & 0.58 & $\checkmark$ & 0.27 \\
9b & $\times$ & 4.33 & $\times$ & 46.24 & $\times$ & 4.02 & 30 & $\checkmark$ & 0.27 & $\checkmark$ & 0.49 & $\checkmark$ & 0.26 & 49a & $\times$ & 7.07 & $\times$ & 89.20 & $\times$ & 6.50 \\
10 & $\checkmark$ & 0.32 & $\checkmark$ & 0.56 & $\checkmark$ & 0.30 & 31 & $\times$ & 22.07 & $\times$ & 180.08 & $\times$ & 21.01 & 49b & $\times$ & 6.53 & $\times$ & 87.98 & $\times$ & 6.13 \\
11a & $\times$ & 5.37 & $\times$ & 49.53 & $\times$ & 5.00 & 32 & $\checkmark$ & 0.13 & $\checkmark$ & 0.26 & $\checkmark$ & 0.13 & 49c & $\times$ & 7.25 & $\times$ & 86.36 & $\times$ & 6.57 \\
11b & $\times$ & 5.37 & $\times$ & 50.05 & $\times$ & 4.98 & 33 & $\checkmark$ & 0.13 & $\checkmark$ & 0.17 & $\times$ & 3.19 & 50 & $\checkmark$ & 0.27 & $\checkmark$ & 0.56 & $\checkmark$ & 0.26 \\
11c & $\times$ & 4.70 & $\times$ & 47.70 & $\times$ & 4.38 & 34 & $\checkmark$ & 0.13 & $\checkmark$ & 0.18 & $\checkmark$ & 0.13 & 51 & $\times$ & 10.08 & $\times$ & 180.07 & $\times$ & 9.19 \\
12 & $\checkmark$ & 0.34 & $\checkmark$ & 9.35 & $\times$ & 3.75 & 35a & $\times$ & 5.65 & $\times$ & 87.32 & $\times$ & 5.64 & 52 & $\checkmark$ & 0.27 & $\checkmark$ & 0.56 & $\checkmark$ & 0.26 \\
13 & $\checkmark$ & 0.08 & $\checkmark$ & 0.16 & $\checkmark$ & 0.04 & 35b & $\times$ & 6.21 & $\times$ & 94.28 & $\times$ & 6.13 & 53 & $\checkmark$ & 0.12 & $\checkmark$ & 0.16 & $\times$ & 3.25 \\
14 & $\times$ & 29.04 & $\times$ & 107.60 & $\times$ & 28.89 & 35c & $\times$ & 6.25 & $\times$ & 90.34 & $\times$ & 6.11 & 54 & $\checkmark$ & 0.13 & $\checkmark$ & 0.18 & $\checkmark$ & 0.13 \\
15 & $\times$ & 113.98 & $\times$ & 166.84 & $\times$ & 118.83 & 36a & $\times$ & 6.11 & $\times$ & 83.95 & $\times$ & 6.04 & 55 & $\times$ & 39.77 & $\times$ & 180.56 & $\times$ & 31.39 \\
16a & $\times$ & 5.50 & $\times$ & 49.60 & $\times$ & 5.11 & 36b & $\times$ & 5.71 & $\times$ & 83.44 & $\times$ & 5.62 & 56 & $\checkmark$ & 0.23 & $\checkmark$ & 0.25 & $\times$ & 3.36 \\
16b & $\times$ & 5.41 & $\times$ & 49.02 & $\times$ & 5.12 & 36c & $\times$ & 6.47 & $\times$ & 84.76 & $\times$ & 6.12 & 57 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 \\
16c & $\times$ & 5.40 & $\times$ & 52.49 & $\times$ & 5.13 & 37 & $\checkmark$ & 0.05 & $\checkmark$ & 0.13 & $\times$ & 2.76 & 58 & $\times$ & 38.92 & $\times$ & 180.14 & $\times$ & 30.91 \\
17 & $\times$ & 180.11 & $\times$ & 199.42 & $\times$ & 180.05 & 38 & $\checkmark$ & 0.05 & $\checkmark$ & 0.06 & $\times$ & 2.77 & 59 & $\checkmark$ & 0.33 & $\checkmark$ & 0.51 & $\checkmark$ & 0.32 \\
18 & $\times$ & 3.16 & $\times$ & 5.49 & $\times$ & 3.00 & 39a & $\times$ & 6.37 & $\times$ & 84.63 & $\times$ & 6.00 & 60 & $\checkmark$ & 0.36 & $\checkmark$ & 0.56 & $\checkmark$ & 0.35 \\
19 & $\checkmark$ & 0.27 & $\checkmark$ & 0.49 & $\times$ & 2.73 & 39b & $\times$ & 5.67 & $\times$ & 83.15 & $\times$ & 5.51 & 61 & $\times$ & 5.66 & $\times$ & 41.94 & $\times$ & 5.21 \\
20 & $\checkmark$ & 0.27 & $\checkmark$ & 0.49 & $\checkmark$ & 0.26 & 39c & $\times$ & 6.39 & $\times$ & 84.98 & $\times$ & 6.10 & 62 & $\times$ & 10.13 & $\times$ & 180.25 & $\times$ & 9.17 \\
21 & $\checkmark$ & 0.28 & $\checkmark$ & 0.50 & $\checkmark$ & 0.26 & 40 & $\checkmark$ & 0.10 & $\checkmark$ & 0.11 & $\checkmark$ & 0.10 & 63 & $\times$ & 10.15 & $\times$ & 180.10 & $\times$ & 9.21 \\
\cline{15-21}
22 & $\checkmark$ & 0.21 & $\checkmark$ & 5.94 & $\checkmark$ & 0.48 & 41 & $\checkmark$ & 0.11 & $\checkmark$ & 0.11 & $\checkmark$ & 0.11 & \textbf{Tot} & \textbf{37} & \textbf{1078.75} & \textbf{37} & \textbf{4932.67} & \textbf{29} & \textbf{1023.70} \\
23 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & 42 & $\checkmark$ & 0.11 & $\checkmark$ & 0.12 & $\checkmark$ & 0.11 &  &  &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
}
    \label{tab:precond_input}
\end{table*}



==> exp/tables/precond_table_weight.tex <==
\begin{table*}[th]
    \centering
    \caption{Detail Results for precondition-fix suggestion for  imposing on  \underline{only weight nodes} for \sysname and baseline approaches~(\sysname-E and GD). ``$\checkmark$'' means precondition that fixes all numerical defects is found and ``$\times$'' means otherwise. ``Time (s)'' is the running time. 
    All approaches are deterministic.}
\resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|cccccc||c|cccccc||c|cccccc}
        \toprule
        \multirow{2}{*}{Case} & \multicolumn{6}{c|}{Impose on Weight} & 
        \multirow{2}{*}{Case} & \multicolumn{6}{c|}{Impose on Weight} &
        \multirow{2}{*}{Case} & \multicolumn{6}{c}{Impose on Weight} \\
        \cline{2-7}
        \cline{9-14}
        \cline{16-21}
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c|}{GD} &
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c|}{GD} &
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c}{GD} \\
        \cline{2-7}
        \cline{9-14}
        \cline{16-21}
        
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s)  \\
        
        \hline

1 & $\checkmark$ & 19.90 & $\checkmark$ & 36.65 & $\checkmark$ & 1.09 & 24 & $\checkmark$ & 1.09 & $\checkmark$ & 26.24 & $\checkmark$ & 0.16 & 43a & $\checkmark$ & 0.18 & $\checkmark$ & 2.91 & $\times$ & 7.97 \\
2a & $\times$ & 3.79 & $\times$ & 17.32 & $\times$ & 4.23 & 25 & $\checkmark$ & 0.25 & $\checkmark$ & 0.84 & $\times$ & 3.29 & 43b & $\checkmark$ & 0.16 & $\checkmark$ & 2.93 & $\checkmark$ & 0.02 \\
2b & $\checkmark$ & 0.42 & $\checkmark$ & 1.80 & $\times$ & 4.15 & 26 & $\checkmark$ & 0.15 & $\checkmark$ & 0.25 & $\times$ & 3.75 & 43c & $\checkmark$ & 0.18 & $\checkmark$ & 2.75 & $\times$ & 7.96 \\
3 & $\checkmark$ & 0.24 & $\checkmark$ & 1.23 & $\times$ & 3.20 & 27 & $\times$ & 0.00 & $\times$ & 0.00 & $\times$ & 0.00 & 44 & $\checkmark$ & 0.98 & $\checkmark$ & 6.84 & $\checkmark$ & 0.17 \\
4 & $\times$ & 0.00 & $\times$ & 0.01 & $\times$ & 0.00 & 28a & $\checkmark$ & 1.28 & $\checkmark$ & 6.20 & $\times$ & 18.93 & 45a & $\checkmark$ & 0.34 & $\checkmark$ & 1.49 & $\checkmark$ & 0.35 \\
5 & $\times$ & 0.00 & $\times$ & 0.01 & $\times$ & 0.01 & 28b & $\checkmark$ & 1.27 & $\checkmark$ & 6.37 & $\times$ & 18.78 & 45b & $\checkmark$ & 1.51 & $\checkmark$ & 33.85 & $\checkmark$ & 0.10 \\
6 & $\checkmark$ & 1.75 & $\checkmark$ & 34.66 & $\checkmark$ & 0.12 & 28c & $\checkmark$ & 0.33 & $\checkmark$ & 1.98 & $\checkmark$ & 0.08 & 46 & $\times$ & 0.00 & $\times$ & 0.00 & $\times$ & 0.00 \\
7 & $\checkmark$ & 1.57 & $\checkmark$ & 34.50 & $\checkmark$ & 0.12 & 28d & $\checkmark$ & 0.06 & $\checkmark$ & 0.30 & $\checkmark$ & 0.02 & 47 & $\checkmark$ & 0.21 & $\checkmark$ & 0.19 & $\checkmark$ & 0.21 \\
8 & $\checkmark$ & 1.57 & $\checkmark$ & 34.49 & $\checkmark$ & 0.12 & 28e & $\checkmark$ & 0.06 & $\checkmark$ & 0.34 & $\checkmark$ & 0.02 & 48a & $\checkmark$ & 0.61 & $\checkmark$ & 5.75 & $\checkmark$ & 0.61 \\
9a & $\checkmark$ & 0.32 & $\checkmark$ & 4.39 & $\times$ & 4.78 & 29 & $\checkmark$ & 1.36 & $\checkmark$ & 26.67 & $\checkmark$ & 0.13 & 48b & $\checkmark$ & 0.27 & $\checkmark$ & 1.52 & $\checkmark$ & 0.26 \\
9b & $\checkmark$ & 0.24 & $\checkmark$ & 4.31 & $\times$ & 4.75 & 30 & $\checkmark$ & 0.27 & $\checkmark$ & 1.43 & $\checkmark$ & 0.27 & 49a & $\checkmark$ & 0.17 & $\checkmark$ & 3.22 & $\times$ & 7.85 \\
10 & $\checkmark$ & 0.26 & $\checkmark$ & 1.44 & $\checkmark$ & 0.26 & 31 & $\checkmark$ & 0.49 & $\checkmark$ & 13.69 & $\times$ & 26.31 & 49b & $\checkmark$ & 0.16 & $\checkmark$ & 3.03 & $\checkmark$ & 0.02 \\
11a & $\checkmark$ & 0.17 & $\checkmark$ & 1.88 & $\checkmark$ & 0.01 & 32 & $\checkmark$ & 0.15 & $\checkmark$ & 0.18 & $\checkmark$ & 0.14 & 49c & $\checkmark$ & 0.18 & $\checkmark$ & 2.66 & $\times$ & 7.98 \\
11b & $\checkmark$ & 0.18 & $\checkmark$ & 1.66 & $\checkmark$ & 0.01 & 33 & $\checkmark$ & 0.14 & $\checkmark$ & 0.16 & $\times$ & 3.57 & 50 & $\checkmark$ & 0.27 & $\checkmark$ & 1.52 & $\checkmark$ & 0.26 \\
11c & $\checkmark$ & 0.15 & $\checkmark$ & 1.72 & $\checkmark$ & 0.01 & 34 & $\checkmark$ & 0.14 & $\checkmark$ & 0.18 & $\checkmark$ & 0.14 & 51 & $\checkmark$ & 0.51 & $\checkmark$ & 15.76 & $\times$ & 11.21 \\
12 & $\checkmark$ & 0.21 & $\checkmark$ & 4.81 & $\checkmark$ & 0.20 & 35a & $\checkmark$ & 0.15 & $\checkmark$ & 2.70 & $\checkmark$ & 0.02 & 52 & $\checkmark$ & 0.27 & $\checkmark$ & 1.49 & $\checkmark$ & 0.27 \\
13 & $\times$ & 0.00 & $\times$ & 0.01 & $\times$ & 0.00 & 35b & $\checkmark$ & 0.17 & $\checkmark$ & 2.84 & $\times$ & 7.75 & 53 & $\checkmark$ & 0.12 & $\checkmark$ & 0.23 & $\times$ & 3.68 \\
14 & $\checkmark$ & 0.89 & $\checkmark$ & 3.17 & $\checkmark$ & 0.06 & 35c & $\checkmark$ & 0.17 & $\checkmark$ & 2.92 & $\times$ & 7.70 & 54 & $\checkmark$ & 0.14 & $\checkmark$ & 0.18 & $\checkmark$ & 0.13 \\
15 & $\checkmark$ & 1.99 & $\checkmark$ & 3.12 & $\checkmark$ & 2.59 & 36a & $\checkmark$ & 0.17 & $\checkmark$ & 2.75 & $\times$ & 7.65 & 55 & $\checkmark$ & 1.52 & $\checkmark$ & 33.66 & $\checkmark$ & 0.10 \\
16a & $\checkmark$ & 0.24 & $\checkmark$ & 1.86 & $\checkmark$ & 0.03 & 36b & $\checkmark$ & 0.15 & $\checkmark$ & 3.20 & $\checkmark$ & 0.02 & 56 & $\checkmark$ & 0.22 & $\checkmark$ & 0.17 & $\times$ & 3.79 \\
16b & $\checkmark$ & 0.18 & $\checkmark$ & 1.67 & $\checkmark$ & 0.02 & 36c & $\checkmark$ & 0.17 & $\checkmark$ & 2.81 & $\times$ & 7.77 & 57 & $\times$ & 0.00 & $\times$ & 0.00 & $\times$ & 0.00 \\
16c & $\checkmark$ & 0.18 & $\checkmark$ & 1.80 & $\checkmark$ & 0.02 & 37 & $\checkmark$ & 0.06 & $\checkmark$ & 0.12 & $\times$ & 3.11 & 58 & $\checkmark$ & 1.52 & $\checkmark$ & 34.48 & $\checkmark$ & 0.13 \\
17 & $\checkmark$ & 4.91 & $\times$ & 211.36 & $\checkmark$ & 0.54 & 38 & $\checkmark$ & 0.06 & $\checkmark$ & 0.07 & $\times$ & 3.12 & 59 & $\checkmark$ & 0.31 & $\checkmark$ & 1.22 & $\checkmark$ & 0.31 \\
18 & $\checkmark$ & 0.25 & $\checkmark$ & 1.11 & $\checkmark$ & 0.25 & 39a & $\checkmark$ & 0.17 & $\checkmark$ & 2.53 & $\times$ & 7.55 & 60 & $\checkmark$ & 0.34 & $\checkmark$ & 1.49 & $\checkmark$ & 0.35 \\
19 & $\checkmark$ & 0.26 & $\checkmark$ & 1.58 & $\times$ & 2.78 & 39b & $\checkmark$ & 0.15 & $\checkmark$ & 2.71 & $\checkmark$ & 0.02 & 61 & $\checkmark$ & 0.53 & $\checkmark$ & 5.10 & $\checkmark$ & 0.53 \\
20 & $\checkmark$ & 0.27 & $\checkmark$ & 1.47 & $\checkmark$ & 0.27 & 39c & $\checkmark$ & 0.17 & $\checkmark$ & 2.89 & $\times$ & 7.67 & 62 & $\checkmark$ & 0.52 & $\checkmark$ & 16.44 & $\times$ & 11.34 \\
21 & $\checkmark$ & 0.27 & $\checkmark$ & 1.50 & $\checkmark$ & 0.27 & 40 & $\checkmark$ & 0.10 & $\checkmark$ & 0.16 & $\checkmark$ & 0.11 & 63 & $\checkmark$ & 0.51 & $\checkmark$ & 15.87 & $\times$ & 11.24 \\
\cline{15-21}
22 & $\checkmark$ & 0.21 & $\checkmark$ & 6.95 & $\checkmark$ & 0.21 & 41 & $\checkmark$ & 0.11 & $\checkmark$ & 0.12 & $\checkmark$ & 0.11 & \textbf{Tot} & \textbf{77} & \textbf{61.15} & \textbf{76} & \textbf{722.00} & \textbf{49} & \textbf{235.21} \\
23 & $\times$ & 0.00 & $\times$ & 0.01 & $\times$ & 0.00 & 42 & $\checkmark$ & 0.11 & $\checkmark$ & 0.12 & $\checkmark$ & 0.11 &  &  &  &  &  &  &  \\


        \bottomrule
    \end{tabular}
}
    \label{tab:precond_weight}
\end{table*}



==> exp/tables/precond_table_weight_input.tex <==
\begin{table*}[th]
    \centering
    \caption{Detail Results for precondition-fix suggestion for  imposing on \underline{both weight and input nodes} for \sysname and baseline approaches~(\sysname-E and GD). ``$\checkmark$'' means precondition that fixes all numerical defects is found and ``$\times$'' means otherwise. ``Time (s)'' is the running time. 
    All approaches are deterministic.}
\resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|cccccc||c|cccccc||c|cccccc}
        \toprule
        \multirow{2}{*}{Case} & \multicolumn{6}{c|}{Impose on Weight + Input} & 
        \multirow{2}{*}{Case} & \multicolumn{6}{c|}{Impose on Weight + Input} &
        \multirow{2}{*}{Case} & \multicolumn{6}{c}{Impose on Weight + Input} \\
        \cline{2-7}
        \cline{9-14}
        \cline{16-21}
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c|}{GD} &
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c|}{GD} &
        \multirow{2}{*}{ID} & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{\sysname-E} & \multicolumn{2}{c}{GD} \\
        \cline{2-7}
        \cline{9-14}
        \cline{16-21}
        
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s) &
         & $\checkmark$/$\times$ & Time (s) & 
        $\checkmark$/$\times$ & Time (s) &
        $\checkmark$/$\times$ & Time (s)  \\
        
        \hline

1 & $\checkmark$ & 20.47 & $\checkmark$ & 38.51 & $\checkmark$ & 1.14 & 24 & $\checkmark$ & 1.10 & $\checkmark$ & 26.36 & $\checkmark$ & 0.10 & 43a & $\checkmark$ & 0.18 & $\checkmark$ & 3.47 & $\times$ & 8.67 \\
2a & $\checkmark$ & 0.30 & $\checkmark$ & 0.90 & $\checkmark$ & 0.44 & 25 & $\checkmark$ & 0.18 & $\checkmark$ & 0.39 & $\checkmark$ & 0.26 & 43b & $\checkmark$ & 0.17 & $\checkmark$ & 2.92 & $\checkmark$ & 0.02 \\
2b & $\checkmark$ & 0.23 & $\checkmark$ & 0.97 & $\checkmark$ & 0.25 & 26 & $\checkmark$ & 0.09 & $\checkmark$ & 0.16 & $\times$ & 4.12 & 43c & $\checkmark$ & 0.18 & $\checkmark$ & 3.16 & $\times$ & 8.87 \\
3 & $\checkmark$ & 0.14 & $\checkmark$ & 0.57 & $\checkmark$ & 0.26 & 27 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & 44 & $\checkmark$ & 0.95 & $\checkmark$ & 7.18 & $\checkmark$ & 0.14 \\
4 & $\checkmark$ & 0.10 & $\checkmark$ & 0.16 & $\checkmark$ & 0.06 & 28a & $\checkmark$ & 0.95 & $\checkmark$ & 4.71 & $\times$ & 18.91 & 45a & $\checkmark$ & 0.24 & $\checkmark$ & 0.77 & $\checkmark$ & 0.26 \\
5 & $\checkmark$ & 0.01 & $\checkmark$ & 0.04 & $\checkmark$ & 0.01 & 28b & $\checkmark$ & 0.94 & $\checkmark$ & 4.95 & $\times$ & 19.29 & 45b & $\checkmark$ & 1.61 & $\checkmark$ & 34.81 & $\checkmark$ & 0.11 \\
6 & $\checkmark$ & 1.58 & $\checkmark$ & 33.70 & $\checkmark$ & 0.13 & 28c & $\checkmark$ & 0.33 & $\checkmark$ & 2.02 & $\checkmark$ & 0.08 & 46 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 \\
7 & $\checkmark$ & 1.69 & $\checkmark$ & 34.95 & $\checkmark$ & 0.11 & 28d & $\checkmark$ & 0.06 & $\checkmark$ & 0.35 & $\checkmark$ & 0.02 & 47 & $\checkmark$ & 0.14 & $\checkmark$ & 0.11 & $\checkmark$ & 0.14 \\
8 & $\checkmark$ & 1.57 & $\checkmark$ & 34.46 & $\checkmark$ & 0.12 & 28e & $\checkmark$ & 0.06 & $\checkmark$ & 0.42 & $\checkmark$ & 0.02 & 48a & $\checkmark$ & 0.37 & $\checkmark$ & 2.93 & $\checkmark$ & 1.04 \\
9a & $\checkmark$ & 0.34 & $\checkmark$ & 4.25 & $\times$ & 5.28 & 29 & $\checkmark$ & 1.25 & $\checkmark$ & 26.72 & $\checkmark$ & 0.12 & 48b & $\checkmark$ & 0.16 & $\checkmark$ & 0.73 & $\checkmark$ & 0.16 \\
9b & $\checkmark$ & 0.26 & $\checkmark$ & 4.43 & $\times$ & 5.26 & 30 & $\checkmark$ & 0.16 & $\checkmark$ & 0.69 & $\checkmark$ & 0.17 & 49a & $\checkmark$ & 0.18 & $\checkmark$ & 3.10 & $\times$ & 8.74 \\
10 & $\checkmark$ & 0.15 & $\checkmark$ & 0.61 & $\checkmark$ & 0.16 & 31 & $\checkmark$ & 0.49 & $\checkmark$ & 14.24 & $\times$ & 28.30 & 49b & $\checkmark$ & 0.17 & $\checkmark$ & 3.16 & $\checkmark$ & 0.02 \\
11a & $\checkmark$ & 0.18 & $\checkmark$ & 2.10 & $\checkmark$ & 0.01 & 32 & $\checkmark$ & 0.08 & $\checkmark$ & 0.11 & $\checkmark$ & 0.09 & 49c & $\checkmark$ & 0.18 & $\checkmark$ & 3.28 & $\times$ & 8.83 \\
11b & $\checkmark$ & 0.18 & $\checkmark$ & 1.84 & $\checkmark$ & 0.01 & 33 & $\checkmark$ & 0.08 & $\checkmark$ & 0.10 & $\times$ & 4.17 & 50 & $\checkmark$ & 0.16 & $\checkmark$ & 0.76 & $\checkmark$ & 0.16 \\
11c & $\checkmark$ & 0.16 & $\checkmark$ & 1.84 & $\checkmark$ & 0.01 & 34 & $\checkmark$ & 0.08 & $\checkmark$ & 0.11 & $\checkmark$ & 0.08 & 51 & $\checkmark$ & 0.28 & $\checkmark$ & 8.97 & $\checkmark$ & 0.84 \\
12 & $\checkmark$ & 0.15 & $\checkmark$ & 3.55 & $\checkmark$ & 0.23 & 35a & $\checkmark$ & 0.16 & $\checkmark$ & 3.24 & $\checkmark$ & 0.02 & 52 & $\checkmark$ & 0.15 & $\checkmark$ & 0.66 & $\checkmark$ & 0.17 \\
13 & $\checkmark$ & 0.08 & $\checkmark$ & 0.17 & $\checkmark$ & 0.05 & 35b & $\checkmark$ & 0.18 & $\checkmark$ & 3.35 & $\times$ & 8.44 & 53 & $\checkmark$ & 0.07 & $\checkmark$ & 0.14 & $\times$ & 4.24 \\
14 & $\checkmark$ & 0.92 & $\checkmark$ & 3.45 & $\checkmark$ & 0.13 & 35c & $\checkmark$ & 0.17 & $\checkmark$ & 3.03 & $\times$ & 8.46 & 54 & $\checkmark$ & 0.08 & $\checkmark$ & 0.11 & $\checkmark$ & 0.08 \\
15 & $\checkmark$ & 1.77 & $\checkmark$ & 2.31 & $\checkmark$ & 2.14 & 36a & $\checkmark$ & 0.17 & $\checkmark$ & 3.27 & $\times$ & 8.28 & 55 & $\checkmark$ & 1.59 & $\checkmark$ & 34.21 & $\checkmark$ & 0.10 \\
16a & $\checkmark$ & 0.26 & $\checkmark$ & 1.94 & $\checkmark$ & 0.03 & 36b & $\checkmark$ & 0.16 & $\checkmark$ & 2.89 & $\checkmark$ & 0.02 & 56 & $\checkmark$ & 0.16 & $\checkmark$ & 0.10 & $\times$ & 4.42 \\
16b & $\checkmark$ & 0.18 & $\checkmark$ & 1.82 & $\checkmark$ & 0.03 & 36c & $\checkmark$ & 0.17 & $\checkmark$ & 3.08 & $\times$ & 8.43 & 57 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 & $\checkmark$ & 0.01 \\
16c & $\checkmark$ & 0.18 & $\checkmark$ & 2.03 & $\checkmark$ & 0.03 & 37 & $\checkmark$ & 0.03 & $\checkmark$ & 0.09 & $\times$ & 3.67 & 58 & $\checkmark$ & 1.61 & $\checkmark$ & 34.13 & $\checkmark$ & 0.12 \\
17 & $\checkmark$ & 4.64 & $\times$ & 215.34 & $\checkmark$ & 0.57 & 38 & $\checkmark$ & 0.03 & $\checkmark$ & 0.04 & $\times$ & 3.63 & 59 & $\checkmark$ & 0.22 & $\checkmark$ & 0.59 & $\checkmark$ & 0.22 \\
18 & $\checkmark$ & 0.16 & $\checkmark$ & 0.56 & $\checkmark$ & 0.16 & 39a & $\checkmark$ & 0.17 & $\checkmark$ & 3.13 & $\times$ & 8.15 & 60 & $\checkmark$ & 0.23 & $\checkmark$ & 0.77 & $\checkmark$ & 0.24 \\
19 & $\checkmark$ & 0.15 & $\checkmark$ & 0.65 & $\times$ & 3.28 & 39b & $\checkmark$ & 0.15 & $\checkmark$ & 3.22 & $\checkmark$ & 0.02 & 61 & $\checkmark$ & 0.31 & $\checkmark$ & 2.93 & $\checkmark$ & 0.89 \\
20 & $\checkmark$ & 0.16 & $\checkmark$ & 0.80 & $\checkmark$ & 0.16 & 39c & $\checkmark$ & 0.17 & $\checkmark$ & 3.01 & $\times$ & 8.33 & 62 & $\checkmark$ & 0.28 & $\checkmark$ & 9.28 & $\checkmark$ & 1.45 \\
21 & $\checkmark$ & 0.15 & $\checkmark$ & 0.68 & $\checkmark$ & 0.16 & 40 & $\checkmark$ & 0.06 & $\checkmark$ & 0.07 & $\checkmark$ & 0.07 & 63 & $\checkmark$ & 0.27 & $\checkmark$ & 9.35 & $\checkmark$ & 2.95 \\
\cline{15-21}
22 & $\checkmark$ & 0.12 & $\checkmark$ & 4.47 & $\checkmark$ & 0.15 & 41 & $\checkmark$ & 0.06 & $\checkmark$ & 0.07 & $\checkmark$ & 0.07 & \textbf{Tot} & \textbf{85} & \textbf{53.86} & \textbf{84} & \textbf{674.67} & \textbf{63} & \textbf{206.64} \\
23 & $\checkmark$ & 0.01 & $\checkmark$ & 0.02 & $\checkmark$ & 0.01 & 42 & $\checkmark$ & 0.07 & $\checkmark$ & 0.07 & $\checkmark$ & 0.07 &  &  &  &  &  &  &  \\


        \bottomrule
    \end{tabular}
}
    \label{tab:precond_weight_input}
\end{table*}


